Builtin Types viewed as Inductive Families

State of the art optimisation passes for dependently typed languages can help erase the redundant information typical of invariant-rich data structures and programs. These automated processes do not dramatically change the structure of the data, even though more efficient representations could be available. Using Quantitative Type Theory, we demonstrate how to define an invariant-rich, typechecking time data structure packing an efficient runtime representation together with runtime irrelevant invariants. The compiler can then aggressively erase all such invariants during compilation. Unlike other approaches, the complexity of the resulting representation is entirely predictable, we do not require both representations to have the same structure, and yet we are able to seamlessly program as if we were using the high-level structure.

==> Data/Bits/Integer.idr.tex <==

\begin{code}
\IdrisKeyword{module}\KatlaSpace{}\IdrisModule{Data.Bits.Integer}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Bits}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisModule{Data.Bits.Integer.Postulated}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Bool}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.So}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Nat.Order}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Syntax.PreorderReasoning}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{\%default}\KatlaSpace{}\IdrisKeyword{total}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Additional\KatlaSpace{}functions}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}cofull\KatlaSpace{}takes\KatlaSpace{}a\KatlaSpace{}natural\KatlaSpace{}number\KatlaSpace{}n\KatlaSpace{}and\KatlaSpace{}returns\KatlaSpace{}an\KatlaSpace{}integer\KatlaSpace{}whose\KatlaSpace{}bit\KatlaSpace{}pattern\KatlaSpace{}is}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}n\KatlaSpace{}zeros\KatlaSpace{}followed\KatlaSpace{}by\KatlaSpace{}ones}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*cofull>
\begin{code}
\IdrisFunction{cofull}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Integer}\KatlaNewline{}
\IdrisFunction{cofull}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{oneBits}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisBound{n}\KatlaNewline{}
\end{code}
%</cofull>
\begin{code}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}full\KatlaSpace{}takes\KatlaSpace{}a\KatlaSpace{}natural\KatlaSpace{}number\KatlaSpace{}n\KatlaSpace{}and\KatlaSpace{}returns\KatlaSpace{}an\KatlaSpace{}integer\KatlaSpace{}whose\KatlaSpace{}bit\KatlaSpace{}pattern\KatlaSpace{}is}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}n\KatlaSpace{}ones\KatlaSpace{}followed\KatlaSpace{}by\KatlaSpace{}zeros}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*full>
\begin{code}
\IdrisFunction{full}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Integer}\KatlaNewline{}
\IdrisFunction{full}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{complement}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cofull}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</full>
\begin{code}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}cons\KatlaSpace{}takes\KatlaSpace{}a\KatlaSpace{}bit\KatlaSpace{}and\KatlaSpace{}an\KatlaSpace{}integer\KatlaSpace{}and\KatlaSpace{}returns\KatlaSpace{}an\KatlaSpace{}integer\KatlaSpace{}whose\KatlaSpace{}bit\KatlaSpace{}pattern}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}is\KatlaSpace{}that\KatlaSpace{}bit\KatlaSpace{}followed\KatlaSpace{}by\KatlaSpace{}the\KatlaSpace{}original\KatlaSpace{}integer}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*cons>
\begin{code}
\IdrisFunction{cons}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Bool}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Integer}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Integer}\KatlaNewline{}
\IdrisFunction{cons}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{bs0}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{if}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{then}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs0}\KatlaSpace{}\IdrisFunction{`setBit`}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{else}\KatlaSpace{}\IdrisBound{bs0}\KatlaNewline{}
\end{code}
%</cons>
\begin{code}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}And\KatlaSpace{}properties}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{shiftRAnd}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.\&.}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisFunction{.\&.}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisBound{k}\KatlaNewline{}
\IdrisFunction{shiftRAnd}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{extensionally}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitAnd}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitShiftR}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitShiftR}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitShiftR}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.\&.}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitAnd}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{andIdempotent}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.\&.}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{bs}\KatlaNewline{}
\IdrisFunction{andIdempotent}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{extensionally}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitAnd}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{andSameNeutral}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}ShiftL\KatlaSpace{}properties}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{shiftLSR}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisBound{k}\KatlaNewline{}
\IdrisFunction{shiftLSR}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{extensionally}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{Calc}\KatlaSpace{}\$\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{|\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{((}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{testBitShiftR}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{testBitSShiftL}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{shiftLR}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{bs}\KatlaNewline{}
\IdrisFunction{shiftLR}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{Calc}\KatlaSpace{}\$\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{|\KatlaTilde{}}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{shiftLSR}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{shiftL0}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{setBit0ShiftR}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{setBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\KatlaNewline{}
\IdrisFunction{setBit0ShiftR}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{extensionally}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{Calc}\KatlaSpace{}\$\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{|\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{setBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{setBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{testBitShiftR}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{setBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{testSetBitOther}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{absurd}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{sym}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{testBitShiftR}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{shiftLInjective}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{cs}\KatlaNewline{}
\IdrisFunction{shiftLInjective}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{Calc}\KatlaSpace{}\$\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{|\KatlaTilde{}}\KatlaSpace{}\IdrisBound{bs}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{sym}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{shiftL0}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{shiftL0}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{shiftLInjective}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{eq}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{shiftLInjective}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{k}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{extensionally}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{Calc}\KatlaSpace{}\$\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{|\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{sym}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{testBitSShiftL}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(\textbackslash{}}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{))}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{testBitSShiftL}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Bit\KatlaSpace{}properties}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{shiftRBitS}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{bit}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisFunction{the}\KatlaSpace{}\IdrisType{Integer}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{bit}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{shiftRBitS}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{shiftLSR}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisBound{i}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Ones\KatlaSpace{}properties}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{testBitOneBits}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{oneBits}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{\})}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisData{True}\KatlaNewline{}
\IdrisFunction{testBitOneBits}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\IdrisFunction{testBitOneBits}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{Calc}\KatlaSpace{}\$\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{|\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{the}\KatlaSpace{}\IdrisType{Integer}\KatlaSpace{}\IdrisFunction{oneBits}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{the}\KatlaSpace{}\IdrisType{Integer}\KatlaSpace{}\IdrisFunction{oneBits}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{sym}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{testBitShiftR}\KatlaSpace{}\IdrisFunction{oneBits}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisData{True}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{testBitOneBits}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Zeros\KatlaSpace{}properties}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{testBitZeroBits}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{zeroBits}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{\})}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisData{False}\KatlaNewline{}
\IdrisFunction{testBitZeroBits}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{Calc}\KatlaSpace{}\$\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{|\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{the}\KatlaSpace{}\IdrisType{Integer}\KatlaSpace{}\IdrisFunction{zeroBits}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{not}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{the}\KatlaSpace{}\IdrisType{Integer}\KatlaSpace{}\IdrisFunction{oneBits}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{testBitComplement}\KatlaSpace{}\IdrisFunction{oneBits}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisData{False}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisFunction{not}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBitOneBits}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Or\KatlaSpace{}properties}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{shiftROr}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.|.}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisFunction{.|.}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{shiftROr}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{extensionally}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitOr}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitShiftR}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitShiftR}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitShiftR}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.|.}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitOr}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{orIdempotent}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.|.}\KatlaSpace{}\IdrisBound{bs}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{bs}\KatlaNewline{}
\IdrisFunction{orIdempotent}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{extensionally}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitOr}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{orSameNeutral}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{orZeroBitsRightIdentity}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.|.}\KatlaSpace{}\IdrisFunction{Bits.zeroBits}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{bs}\KatlaNewline{}
\IdrisFunction{orZeroBitsRightIdentity}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{extensionally}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitOr}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{zeroBits}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitZeroBits}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{orFalseNeutral}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{orZeroBitsLeftIdentity}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{Bits.zeroBits}\KatlaSpace{}\IdrisFunction{.|.}\KatlaSpace{}\IdrisBound{bs}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{bs}\KatlaNewline{}
\IdrisFunction{orZeroBitsLeftIdentity}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{extensionally}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitOr}\KatlaSpace{}\IdrisFunction{zeroBits}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitZeroBits}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Complement\KatlaSpace{}properties}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{complementInvolutive}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{complement}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{complement}\KatlaSpace{}\IdrisBound{bs}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{bs}\KatlaNewline{}
\IdrisFunction{complementInvolutive}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{extensionally}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitComplement}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{complement}\KatlaSpace{}\IdrisBound{bs}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitComplement}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{notInvolutive}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Eq\KatlaSpace{}properties}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisFunction{equalNatSound}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{==}\KatlaSpace{}\IdrisBound{j}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{equalNatSound}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Oh}\KatlaNewline{}
\IdrisFunction{equalNatSound}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{j}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{equalNatSound}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cong}\KatlaSpace{}\IdrisFunction{pred}\KatlaSpace{}\IdrisBound{eq}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{equalNatComplete}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{==}\KatlaSpace{}\IdrisBound{j}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{j}\KatlaNewline{}
\IdrisFunction{equalNatComplete}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\IdrisFunction{equalNatComplete}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{j}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{hyp}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{equalNatComplete}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisBound{hyp}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Bit\KatlaSpace{}properties}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{testOneS}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{the}\KatlaSpace{}\IdrisType{Integer}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisData{False}\KatlaNewline{}
\IdrisFunction{testOneS}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\IdrisFunction{testOneS}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{Calc}\KatlaSpace{}\$\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{|\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{2}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{the}\KatlaSpace{}\IdrisType{Integer}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{sym}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{testBitShiftR}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisData{Refl}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisData{False}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{testBitZeroBits}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{testBitBitSame}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{bit}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisData{True}\KatlaNewline{}
\IdrisFunction{testBitBitSame}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{andIdempotent}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{bit}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{bitNonZero}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Constant\KatlaSpace{}properties}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisFunction{notSoToSoNot}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Bool}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{Not}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{So}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{not}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{notSoToSoNot}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{False}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Oh}\KatlaNewline{}
\IdrisFunction{notSoToSoNot}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{True}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{notSo}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{absurd}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{notSo}\KatlaSpace{}\IdrisData{Oh}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}(Co)Full\KatlaSpace{}properties}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{testBitCofull}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cofull}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisFunction{not}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{`lt`}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{testBitCofull}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{testBitOneBits}\KatlaSpace{}\IdrisBound{i}\KatlaNewline{}
\IdrisFunction{testBitCofull}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{testBit0ShiftL}\KatlaSpace{}\IdrisFunction{oneBits}\KatlaSpace{}\IdrisBound{k}\KatlaNewline{}
\IdrisFunction{testBitCofull}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitSShiftL}\KatlaSpace{}\IdrisFunction{oneBits}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{testBitCofull}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{i}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{testBitFull}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{full}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{`lt`}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{testBitFull}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{i}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitComplement}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cofull}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitCofull}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{notInvolutive}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{`lt`}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{shiftRFull}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{full}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisFunction{full}\KatlaSpace{}\IdrisBound{k}\KatlaNewline{}
\IdrisFunction{shiftRFull}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{extensionally}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitShiftR}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{full}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{))}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitFull}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{testBitFull}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}TestBit\KatlaSpace{}properties}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{testSetBitSame}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{setBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{testSetBitSame}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitOr}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{bit}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitBitSame}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{orTrueTrue}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Oh}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Cons\KatlaSpace{}properties}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*testBit0Cons>
\begin{code}
\IdrisFunction{testBit0Cons}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Bool}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cons}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisBound{bs}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{b}\KatlaNewline{}
\end{code}
%</testBit0Cons>
\begin{code}
\IdrisFunction{testBit0Cons}\KatlaSpace{}\IdrisData{True}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{soToEq}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{testSetBitSame}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\KatlaNewline{}
\IdrisFunction{testBit0Cons}\KatlaSpace{}\IdrisData{False}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{testBit0ShiftL}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{0}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{testBitSCons}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Bool}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cons}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisBound{bs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\KatlaNewline{}
\IdrisFunction{testBitSCons}\KatlaSpace{}\IdrisData{True}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{Calc}\KatlaSpace{}\$\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{|\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cons}\KatlaSpace{}\IdrisData{True}\KatlaSpace{}\IdrisBound{bs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{testSetBitOther}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{absurd}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{testBitSShiftL}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(\textbackslash{}}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{shiftL0}\KatlaSpace{}\IdrisBound{bs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{testBitSCons}\KatlaSpace{}\IdrisData{False}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{Calc}\KatlaSpace{}\$\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{|\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cons}\KatlaSpace{}\IdrisData{False}\KatlaSpace{}\IdrisBound{bs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{testBitSShiftL}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(\textbackslash{}}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{shiftL0}\KatlaSpace{}\IdrisBound{bs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*consShiftR>
\begin{code}
\IdrisFunction{consShiftR}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Bool}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cons}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisBound{bs}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{bs}\KatlaNewline{}
\end{code}
%</consShiftR>
\begin{code}
\IdrisFunction{consShiftR}\KatlaSpace{}\IdrisData{True}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Calc}\KatlaSpace{}\$\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{|\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{cons}\KatlaSpace{}\IdrisData{True}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{setBit0ShiftR}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{shiftLR}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{consShiftR}\KatlaSpace{}\IdrisData{False}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{Calc}\KatlaSpace{}\$\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{|\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{cons}\KatlaSpace{}\IdrisData{False}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{shiftLR}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{consInjective}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Bool}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{cons}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisFunction{cons}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{cs}\KatlaNewline{}
\IdrisFunction{consInjective}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{Calc}\KatlaSpace{}\$\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{|\KatlaTilde{}}\KatlaSpace{}\IdrisBound{bs}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{cons}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{sym}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{consShiftR}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisFunction{cons}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{...}\IdrisKeyword{(}\KatlaSpace{}\IdrisFunction{consShiftR}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{)}\KatlaNewline{}
\end{code}



==> Data/Bits/Integer/Postulated.idr.tex <==

\begin{code}
\IdrisComment{|||\KatlaSpace{}Postulated\KatlaSpace{}properties\KatlaSpace{}of\KatlaSpace{}Data.Bits\KatlaSpace{}for\KatlaSpace{}Integer}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}NB:\KatlaSpace{}some\KatlaSpace{}of\KatlaSpace{}these\KatlaSpace{}are\KatlaSpace{}probably\KatlaSpace{}provable}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{module}\KatlaSpace{}\IdrisModule{Data.Bits.Integer.Postulated}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Bits}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Decidable.Equality}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{\%default}\KatlaSpace{}\IdrisKeyword{total}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}This\KatlaSpace{}should\KatlaSpace{}be\KatlaSpace{}far\KatlaSpace{}safer\KatlaSpace{}than\KatlaSpace{}`believe\KatlaUnderscore{}me`\KatlaSpace{}as:}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}1.\KatlaSpace{}we\KatlaSpace{}only\KatlaSpace{}reduce\KatlaSpace{}to\KatlaSpace{}`Refl`\KatlaSpace{}when\KatlaSpace{}x\KatlaSpace{}actually\KatlaSpace{}equals\KatlaSpace{}y}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}2.\KatlaSpace{}we\KatlaSpace{}don't\KatlaSpace{}expose\KatlaSpace{}the\KatlaSpace{}implementation\KatlaSpace{}so\KatlaSpace{}that\KatlaSpace{}users\KatlaSpace{}can't\KatlaSpace{}force\KatlaSpace{}reductions\KatlaSpace{}in\KatlaSpace{}an\KatlaSpace{}absurd\KatlaSpace{}context}\KatlaNewline{}
\IdrisFunction{unsafeRefl}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{DecEq}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{x}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{y}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{y}\KatlaNewline{}
\IdrisFunction{unsafeRefl}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{x}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{y}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{decEq}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisBound{y}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Yes}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{eq}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{No}\KatlaSpace{}\IdrisBound{neq}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisPostulate{assert\KatlaUnderscore{}total}\KatlaSpace{}\$\KatlaSpace{}\IdrisPostulate{idris\KatlaUnderscore{}crash}\KatlaSpace{}\IdrisData{"Equality\KatlaSpace{}postulated\KatlaSpace{}using\KatlaSpace{}unsafeRefl\KatlaSpace{}is\KatlaSpace{}incorrect"}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Extensional\KatlaSpace{}equality}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{infix}\KatlaSpace{}\IdrisKeyword{6}\KatlaSpace{}\KatlaTilde{}\KatlaTilde{}\KatlaTilde{}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*extensionalEq>
\begin{code}
\IdrisFunction{(\KatlaTilde{}\KatlaTilde{}\KatlaTilde{})}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Integer}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Type}\KatlaNewline{}
\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{\KatlaTilde{}\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{i}\KatlaNewline{}
\end{code}
%</extensionalEq>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*extensionally>
\begin{code}
\IdrisFunction{extensionally}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{bs}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{\KatlaTilde{}\KatlaTilde{}\KatlaTilde{}}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{cs}\KatlaNewline{}
\end{code}
%</extensionally>
\begin{code}
\IdrisFunction{extensionally}\KatlaSpace{}\IdrisBound{fext}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{unsafeRefl}\KatlaNewline{}
\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Postulated\KatlaSpace{}properties}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*testBitShiftR>
\begin{code}
\IdrisFunction{testBitShiftR}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</testBitShiftR>
\begin{code}
\IdrisFunction{testBitShiftR}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{unsafeRefl}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*testBit0ShiftL>
\begin{code}
\IdrisFunction{testBit0ShiftL}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisData{False}\KatlaNewline{}
\end{code}
%</testBit0ShiftL>
\begin{code}
\IdrisFunction{testBit0ShiftL}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{unsafeRefl}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\KatlaNewline{}
\end{code}
%<*testBitSShiftL>
\begin{code}
\IdrisFunction{testBitSShiftL}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaNewline{}
\end{code}
%</testBitSShiftL>
\begin{code}
\IdrisFunction{testBitSShiftL}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{unsafeRefl}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*shiftL0>
\begin{code}
\IdrisFunction{shiftL0}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{bs}\KatlaNewline{}
\end{code}
%</shiftL0>
\begin{code}
\IdrisFunction{shiftL0}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{unsafeRefl}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}Postulated:\KatlaSpace{}conjunction\KatlaSpace{}is\KatlaSpace{}bitwise\KatlaSpace{}on\KatlaSpace{}integers}\KatlaNewline{}
\end{code}
%<*testBitAnd>
\begin{code}
\IdrisFunction{testBitAnd}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.\&.}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{\&\&}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</testBitAnd>
\begin{code}
\IdrisFunction{testBitAnd}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{unsafeRefl}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}Postulated:\KatlaSpace{}disjunction\KatlaSpace{}is\KatlaSpace{}bitwise\KatlaSpace{}on\KatlaSpace{}integers}\KatlaNewline{}
\end{code}
%<*testBitOr>
\begin{code}
\IdrisFunction{testBitOr}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.|.}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{||}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</testBitOr>
\begin{code}
\IdrisFunction{testBitOr}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{unsafeRefl}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*testSetBitOther>
\begin{code}
\IdrisFunction{testSetBitOther}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{Not}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{j}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{setBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{j}\KatlaNewline{}
\end{code}
%</testSetBitOther>
\begin{code}
\IdrisFunction{testSetBitOther}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisBound{neq}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{unsafeRefl}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}Postulated:\KatlaSpace{}complement\KatlaSpace{}is\KatlaSpace{}bitwise\KatlaSpace{}on\KatlaSpace{}integers}\KatlaNewline{}
\end{code}
%<*testBitComplement>
\begin{code}
\IdrisFunction{testBitComplement}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{complement}\KatlaSpace{}\IdrisBound{bs}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisFunction{not}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</testBitComplement>
\begin{code}
\IdrisFunction{testBitComplement}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{unsafeRefl}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*bitNonZero>
\begin{code}
\IdrisFunction{bitNonZero}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{bit}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{==}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisData{False}\KatlaNewline{}
\end{code}
%</bitNonZero>
\begin{code}
\IdrisFunction{bitNonZero}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{unsafeRefl}\KatlaNewline{}
\end{code}



==> FinAsNat.idr.tex <==

\begin{code}
\IdrisKeyword{module}\KatlaSpace{}\IdrisModule{FinAsNat}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Nat}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Nat.Order}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{\%default}\KatlaSpace{}\IdrisKeyword{total}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*fin>
\begin{code}
\IdrisKeyword{record}\KatlaSpace{}\IdrisType{Fin}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}constructor\KatlaSpace{}\IdrisData{MkFin}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{encoding}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisFunction{valid}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{encoding}\KatlaSpace{}\IdrisFunction{`LT`}\KatlaSpace{}\IdrisBound{n}\KatlaNewline{}
\end{code}
%</fin>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Smart}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*zero>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Z}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Fin}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Z}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkFin}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{LTESucc}\KatlaSpace{}\IdrisData{LTEZero}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</zero>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*suc>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{S}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Fin}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Fin}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{S}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkFin}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{prf}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkFin}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{LTESucc}\KatlaSpace{}\IdrisBound{prf}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</suc>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*dataview>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{View}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Fin}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{View}\KatlaSpace{}\IdrisFunction{Z}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Fin}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{View}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</dataview>
\begin{code}
\KatlaNewline{}
\IdrisFunction{irrelevantLTE}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{p}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{q}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{LTE}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{q}\KatlaNewline{}
\IdrisFunction{irrelevantLTE}\KatlaSpace{}\IdrisData{LTEZero}\KatlaSpace{}\IdrisData{LTEZero}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\IdrisFunction{irrelevantLTE}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{LTESucc}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{LTESucc}\KatlaSpace{}\IdrisBound{q}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisData{LTESucc}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{irrelevantLTE}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{q}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Smart}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*view>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Fin}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{View}\KatlaSpace{}\IdrisBound{k}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkFin}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{LTESucc}\KatlaSpace{}\IdrisBound{prf}\IdrisKeyword{))}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{irrelevantLTE}\KatlaSpace{}\IdrisBound{prf}\KatlaSpace{}\IdrisData{LTEZero}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisData{Z}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkFin}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{LTESucc}\KatlaSpace{}\IdrisBound{prf}\IdrisKeyword{))}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkFin}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisBound{prf}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</view>
\begin{code}



==> Lookup.idr.tex <==

\begin{code}
\IdrisKeyword{\%default}\KatlaSpace{}\IdrisKeyword{total}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Data}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*vect>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Nil}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{(::)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\end{code}
%</vect>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*fin>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Fin}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Fin}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Fin}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Fin}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</fin>

\begin{code}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Vect}\KatlaNewline{}
\end{code}

%<*vectlookup>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{lookup}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Fin}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{lookup}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{})}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{lookup}\KatlaSpace{}\IdrisKeyword{(\KatlaUnderscore{}}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{lookup}\KatlaSpace{}\IdrisBound{xs}\KatlaSpace{}\IdrisBound{k}\KatlaNewline{}
\end{code}
%</vectlookup>

\begin{code}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{ErasedVect}\KatlaNewline{}
\end{code}

%<*erasedvectlookup>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{partial}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{lookup}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{List}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Nat}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{lookup}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{})}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{lookup}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(\KatlaUnderscore{}}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{lookup}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisBound{xs}\KatlaSpace{}\IdrisBound{k}\KatlaNewline{}
\end{code}
%</erasedvectlookup>

\begin{code}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{List}\KatlaNewline{}
\end{code}

%<*finallookup>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{partial}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{lookup}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{List}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Nat}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{lookup}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{})}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{lookup}\KatlaSpace{}\IdrisKeyword{(\KatlaUnderscore{}}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{lookup}\KatlaSpace{}\IdrisBound{xs}\KatlaSpace{}\IdrisBound{k}\KatlaNewline{}
\end{code}
%</finallookup>



==> LookupRefactor.idr.tex <==

\begin{code}
\IdrisKeyword{module}\KatlaSpace{}\IdrisModule{LookupRefactor}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{VectAsList}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{FinAsNat}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{\%default}\KatlaSpace{}\IdrisKeyword{total}\KatlaNewline{}
\KatlaNewline{}
\end{code}
%<*lookup>
\begin{code}
\IdrisFunction{lookup}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Fin}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\IdrisFunction{lookup}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{@\KatlaUnderscore{}}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{@\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisBound{hd}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{hd}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{tl}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisBound{k'}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{lookup}\KatlaSpace{}\IdrisBound{tl}\KatlaSpace{}\IdrisBound{k'}\KatlaNewline{}
\end{code}
%</lookup>



==> QuantitativeTT.idr.tex <==

\begin{code}
\IdrisKeyword{\%default}\KatlaSpace{}\IdrisKeyword{total}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Typing}\KatlaNewline{}
\end{code}
%<*identity>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{id}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{id}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\end{code}
%</identity>

%<*invalididentity>
\begin{code}
\IdrisKeyword{failing}\KatlaSpace{}\IdrisData{"x\KatlaSpace{}is\KatlaSpace{}not\KatlaSpace{}accessible\KatlaSpace{}in\KatlaSpace{}this\KatlaSpace{}context."}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{id}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{id}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}x\KatlaNewline{}
\end{code}
%</invalididentity>

%<*vect>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}Nat\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Nil}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}Vect\KatlaSpace{}\IdrisData{0}\KatlaSpace{}a\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{(::)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}Nat\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}a\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}Vect\KatlaSpace{}n\KatlaSpace{}a\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}Vect\KatlaSpace{}\IdrisKeyword{(}\IdrisData{1}\KatlaSpace{}+\KatlaSpace{}n\IdrisKeyword{)}\KatlaSpace{}a\KatlaNewline{}
\end{code}
%</vect>


%<*so>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Bool}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Oh}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisData{True}\KatlaNewline{}
\end{code}
%</so>

%<*even>
\begin{code}
\IdrisKeyword{record}\KatlaSpace{}\IdrisType{Even}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}constructor\KatlaSpace{}\IdrisData{MkEven}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{half}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{auto}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisFunction{prf}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{2}\IdrisFunction{\KatlaSpace{}*\KatlaSpace{}}\IdrisBound{half}\IdrisFunction{\KatlaSpace{}==\KatlaSpace{}n}\IdrisKeyword{)\}}\KatlaNewline{}
\end{code}
%</even>

%<*four>
\begin{code}
\IdrisFunction{even6}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Even}\KatlaSpace{}\IdrisData{6}\KatlaNewline{}
\IdrisFunction{even6}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkEven}\KatlaSpace{}\IdrisKeyword{\{}\KatlaSpace{}\IdrisBound{half}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{3}\KatlaSpace{}\IdrisKeyword{\}}\KatlaNewline{}
\end{code}
%</four>



==> Snoc.idr.tex <==

%<*AsSnoc>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{AsSnoc}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{List}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Lin}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{AsSnoc}\KatlaSpace{}\IdrisData{[]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{(:<)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{xs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{List}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{AsSnoc}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{xs}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisData{[}\IdrisBound{x}\IdrisData{]}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</AsSnoc>

%<*asSnoc>
\begin{code}
\IdrisFunction{asSnoc}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{xs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{List}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{AsSnoc}\KatlaSpace{}\IdrisBound{xs}\KatlaNewline{}
\IdrisFunction{asSnoc}\KatlaSpace{}\IdrisData{[]}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{[<]}\KatlaNewline{}
\IdrisFunction{asSnoc}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{asSnoc}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{asSnoc}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisKeyword{.(}\IdrisData{[]}\IdrisKeyword{))}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{[<]}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{[]}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{asSnoc}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisKeyword{.(}\IdrisBound{ys}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisData{[}\IdrisBound{y}\IdrisData{]}\IdrisKeyword{))}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisBound{ys}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{y}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{ys}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{y}\KatlaNewline{}
\end{code}
%</asSnoc>

%<*first>
\begin{code}
\IdrisFunction{first}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{List}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Maybe}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\KatlaNewline{}
\IdrisFunction{first}\KatlaSpace{}\IdrisData{[]}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Nothing}\KatlaNewline{}
\IdrisFunction{first}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{})}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Just}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\end{code}
%</first>

%<*last>
\begin{code}
\IdrisFunction{last}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{List}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Maybe}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\IdrisFunction{last}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{@\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{asSnoc}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{[<]}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Nothing}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisKeyword{(\KatlaUnderscore{}}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Just}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\end{code}
%</last>



==> Thin.idr.tex <==

\begin{code}
\IdrisKeyword{module}\KatlaSpace{}\IdrisModule{Thin}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Bool.Decidable}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Bits}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Bits.Integer}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.DPair}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.SnocList}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.SnocList.Quantifiers}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Decidable.Equality}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Thin.Internal}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{\%default}\KatlaSpace{}\IdrisKeyword{total}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Type\KatlaSpace{}and\KatlaSpace{}interfaces}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}A\KatlaSpace{}Th\KatlaSpace{}is\KatlaSpace{}a\KatlaSpace{}thin\KatlaSpace{}wrapper\KatlaSpace{}around\KatlaSpace{}Invariant\KatlaSpace{}that\KatlaSpace{}only\KatlaSpace{}keeps\KatlaSpace{}the}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}minimal\KatlaSpace{}amount\KatlaSpace{}of\KatlaSpace{}information\KatlaSpace{}as\KatlaSpace{}runtime\KatlaSpace{}relevant.}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*thin>
\begin{code}
\IdrisKeyword{record}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sx}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}constructor\KatlaSpace{}\IdrisData{MkTh}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{bigEnd}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{encoding}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisFunction{invariant}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisBound{bigEnd}\KatlaSpace{}\IdrisBound{encoding}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\KatlaNewline{}
\end{code}
%</thin>
\begin{code}
\IdrisKeyword{\%name}\KatlaSpace{}Th\KatlaSpace{}\IdrisBound{th}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{ps}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{infixr}\KatlaSpace{}\IdrisKeyword{10}\KatlaSpace{}*^\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\IdrisKeyword{interface}\KatlaSpace{}\IdrisType{Thable}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{(*^)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{sa}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{sb}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisBound{sa}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sa}\KatlaSpace{}\IdrisBound{sb}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisBound{sb}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{infixr}\KatlaSpace{}\IdrisKeyword{10}\KatlaSpace{}^?\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\IdrisKeyword{interface}\KatlaSpace{}\IdrisType{Selable}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{(^?)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{sa}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{sb}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sa}\KatlaSpace{}\IdrisBound{sb}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisBound{sb}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{t}\KatlaSpace{}\IdrisBound{sa}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Smart\KatlaSpace{}constructors}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}We\KatlaSpace{}define\KatlaSpace{}the\KatlaSpace{}smart\KatlaSpace{}constructors,\KatlaSpace{}deconstructors,\KatlaSpace{}combinators,\KatlaSpace{}etc.\KatlaSpace{}in\KatlaSpace{}a}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}nested\KatlaSpace{}namespace\KatlaSpace{}so\KatlaSpace{}that\KatlaSpace{}these\KatlaSpace{}definitions\KatlaSpace{}do\KatlaSpace{}not\KatlaSpace{}unfold\KatlaSpace{}in\KatlaSpace{}goals\KatlaSpace{}in\KatlaSpace{}the}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}main\KatlaSpace{}file.\KatlaSpace{}The\KatlaSpace{}eager\KatlaSpace{}unfolding\KatlaSpace{}made\KatlaSpace{}goals\KatlaSpace{}unreadable.}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}We\KatlaSpace{}will\KatlaSpace{}instead\KatlaSpace{}use\KatlaSpace{}the\KatlaSpace{}unfolding\KatlaSpace{}and\KatlaSpace{}irrelevance\KatlaSpace{}lemmas\KatlaSpace{}proved\KatlaSpace{}in\KatlaSpace{}the}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}nested\KatlaSpace{}namespace\KatlaSpace{}to\KatlaSpace{}step\KatlaSpace{}things\KatlaSpace{}when\KatlaSpace{}*we*\KatlaSpace{}need\KatlaSpace{}them\KatlaSpace{}to\KatlaSpace{}step.}\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Smart}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*done>
\begin{code}
\KatlaSpace{}\IdrisFunction{done}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisData{[<]}\KatlaSpace{}\IdrisData{[<]}\KatlaNewline{}
\KatlaSpace{}\IdrisFunction{done}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkTh}\KatlaSpace{}\IdrisKeyword{\{}\KatlaSpace{}\IdrisBound{bigEnd}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{encoding}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{invariant}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{\}}\KatlaNewline{}
\end{code}
%</done>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*keep>
\begin{code}
\KatlaSpace{}\IdrisFunction{keep}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sx}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sy}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\IdrisFunction{keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkTh}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{}\KatlaSpace{}\IdrisBound{bigEnd}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{.bigEnd}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{encoding}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{cons}\KatlaSpace{}\IdrisData{True}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{.encoding}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{invariant}\KatlaSpace{}\IdrisKeyword{=}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{eqToSo}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{testBit0Cons}\KatlaSpace{}\IdrisData{True}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{.encoding}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{consShiftR}\KatlaSpace{}\IdrisData{True}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{.encoding}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{th}\IdrisFunction{.invariant}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\}}\KatlaNewline{}
\end{code}
%</keep>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*drop>
\begin{code}
\KatlaSpace{}\IdrisFunction{drop}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sy}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\IdrisFunction{drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkTh}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{}\KatlaSpace{}\IdrisBound{bigEnd}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{.bigEnd}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{encoding}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{cons}\KatlaSpace{}\IdrisData{False}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{.encoding}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{invariant}\KatlaSpace{}\IdrisKeyword{=}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{prf}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{testBit0Cons}\KatlaSpace{}\IdrisData{False}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{.encoding}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{nb}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{eqToSo}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisFunction{not}\KatlaSpace{}\IdrisBound{prf}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{consShiftR}\KatlaSpace{}\IdrisData{False}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{.encoding}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{.invariant}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\IdrisKeyword{\}}\KatlaNewline{}
\end{code}
%</drop>
\begin{code}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Smart\KatlaSpace{}destructor\KatlaSpace{}(aka\KatlaSpace{}view)}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*view>
\begin{code}
\KatlaSpace{}\IdrisKeyword{data}\KatlaSpace{}\IdrisType{View}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{View}\KatlaSpace{}\IdrisFunction{done}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{View}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{View}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</view>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\IdrisFunction{cast}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisBound{th}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{th'}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{View}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{th}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{View}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{th'}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\IdrisFunction{cast}\KatlaSpace{}\IdrisBound{v}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{replace}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisType{View}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{th}\IdrisKeyword{)\}}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{irrelevantInvariant}\KatlaSpace{}?\KatlaSpace{}?\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{v}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\IdrisKeyword{export}\KatlaSpace{}\IdrisKeyword{\%inline}\KatlaNewline{}
\end{code}
%<*viewtotal>
\begin{code}
\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{View}\KatlaSpace{}\IdrisBound{th}\KatlaNewline{}
\end{code}
%</viewtotal>
%<*viewDone>
\begin{code}
\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{prf}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{eqs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{isDone}\KatlaSpace{}\IdrisBound{prf}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{bsIsZero}\KatlaSpace{}\IdrisBound{eqs}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{fstIndexIsLin}\KatlaSpace{}\IdrisBound{eqs}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{sndIndexIsLin}\KatlaSpace{}\IdrisBound{eqs}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{invariantIsDone}\KatlaSpace{}\IdrisBound{eqs}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Done}\KatlaNewline{}
\end{code}
%</viewDone>
%<*viewKeepDrop>
\begin{code}
\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{prf}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{choose}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{Z}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\end{code}
%</viewKeepDrop>
%<*viewKeep>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Left}\KatlaSpace{}\IdrisBound{so}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{eqs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{isKeep}\KatlaSpace{}\IdrisBound{prf}\KatlaSpace{}\IdrisBound{so}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{fstIndexIsSnoc}\KatlaSpace{}\IdrisBound{eqs}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{sndIndexIsSnoc}\KatlaSpace{}\IdrisBound{eqs}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{invariantIsKeep}\KatlaSpace{}\IdrisBound{eqs}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{isKeepInteger}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{so}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisFunction{th}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{eqs}\IdrisFunction{.fstIndexTail}\KatlaSpace{}\IdrisBound{eqs}\IdrisFunction{.sndIndexTail}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{th}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{eqs}\IdrisFunction{.subInvariant}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{cast}\KatlaSpace{}\$\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisFunction{th}\KatlaSpace{}\IdrisBound{eqs}\IdrisFunction{.keptHead}\KatlaNewline{}
\end{code}
%</viewKeep>
%<*viewDrop>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Right}\KatlaSpace{}\IdrisBound{soNot}\KatlaSpace{}\IdrisKeyword{=>}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{eqs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{isDrop}\KatlaSpace{}\IdrisBound{prf}\KatlaSpace{}\IdrisBound{soNot}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{sndIndexIsSnoc}\KatlaSpace{}\IdrisBound{eqs}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{invariantIsDrop}\KatlaSpace{}\IdrisBound{eqs}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{isDropInteger}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{soNot}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisFunction{th}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{eqs}\IdrisFunction{.sndIndexTail}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{th}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{eqs}\IdrisFunction{.subInvariant}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{cast}\KatlaSpace{}\$\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisFunction{th}\KatlaSpace{}\IdrisBound{eqs}\IdrisFunction{.keptHead}\KatlaNewline{}
\end{code}
%</viewDrop>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Example\KatlaSpace{}of\KatlaSpace{}a\KatlaSpace{}use\KatlaSpace{}of\KatlaSpace{}`view`}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}|||\KatlaSpace{}@\KatlaSpace{}sx\KatlaSpace{}is\KatlaSpace{}runtime\KatlaSpace{}irrelevant\KatlaSpace{}and\KatlaSpace{}yet\KatlaSpace{}we\KatlaSpace{}can\KatlaSpace{}compute\KatlaSpace{}its\KatlaSpace{}length\KatlaSpace{}because}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}|||\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}it\KatlaSpace{}is\KatlaSpace{}precisely\KatlaSpace{}the\KatlaSpace{}number\KatlaSpace{}of\KatlaSpace{}Keep\KatlaSpace{}constructors\KatlaSpace{}(aka\KatlaSpace{}bits\KatlaSpace{}set\KatlaSpace{}to\KatlaSpace{}1)}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}|||\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}in\KatlaSpace{}the\KatlaSpace{}invariant\KatlaSpace{}that\KatlaSpace{}we\KatlaSpace{}have.}\KatlaNewline{}
\end{code}
%<*kept>
\begin{code}
\KatlaSpace{}\IdrisFunction{kept}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{(}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\KatlaSpace{}\IdrisType{**}\KatlaSpace{}\IdrisFunction{length}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{n}\IdrisType{)}\KatlaNewline{}
\KatlaSpace{}\IdrisFunction{kept}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}(\IdrisData{0}\KatlaSpace{}\IdrisData{**}\KatlaSpace{}\IdrisData{Refl})\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}(\IdrisBound{n}\KatlaSpace{}\IdrisData{**}\KatlaSpace{}\IdrisBound{eq})\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{kept}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}(\IdrisData{S}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisData{**}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisBound{eq})\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{kept}\KatlaSpace{}\IdrisBound{th}\KatlaNewline{}
\end{code}
%</kept>
\begin{code}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Unfold\KatlaSpace{}lemmas\KatlaSpace{}for\KatlaSpace{}the\KatlaSpace{}view}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\IdrisFunction{chooseTrueUnfold}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{choose}\KatlaSpace{}\IdrisData{True}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisData{Left}\KatlaSpace{}\IdrisData{Oh}\KatlaNewline{}
\KatlaSpace{}\IdrisFunction{chooseTrueUnfold}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{choose}\KatlaSpace{}\IdrisData{True}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Left}\KatlaSpace{}\IdrisData{Oh}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Right}\KatlaSpace{}\IdrisBound{ohno}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{absurd}\KatlaSpace{}\IdrisBound{ohno}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\IdrisFunction{chooseFalseUnfold}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{choose}\KatlaSpace{}\IdrisData{False}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisData{Right}\KatlaSpace{}\IdrisData{Oh}\KatlaNewline{}
\KatlaSpace{}\IdrisFunction{chooseFalseUnfold}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{choose}\KatlaSpace{}\IdrisData{False}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Left}\KatlaSpace{}\IdrisBound{ohyes}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{absurd}\KatlaSpace{}\IdrisBound{ohyes}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Right}\KatlaSpace{}\IdrisData{Oh}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\IdrisFunction{viewDoneUnfold}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisFunction{done}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisData{Done}\KatlaNewline{}
\KatlaSpace{}\IdrisFunction{viewDoneUnfold}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\IdrisFunction{viewKeepUnfold}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\IdrisFunction{viewKeepUnfold}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBit0Cons}\KatlaSpace{}\IdrisData{True}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{chooseTrueUnfold}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{consShiftR}\KatlaSpace{}\IdrisData{True}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\IdrisFunction{viewDropUnfold}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\IdrisFunction{viewDropUnfold}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBit0Cons}\KatlaSpace{}\IdrisData{False}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{chooseFalseUnfold}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{consShiftR}\KatlaSpace{}\IdrisData{False}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{irrelevantDone}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisData{[<]}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{ph}\KatlaNewline{}
\IdrisFunction{irrelevantDone}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Instances}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisType{Thable}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisBound{th}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{drop}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{keep}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{drop}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisType{Selable}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{`Th`}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{(^?)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{(*^)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisType{Eq}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisFunction{==}\KatlaSpace{}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{==}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisFunction{\&\&}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{==}\KatlaSpace{}\IdrisBound{cs}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisType{Show}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{show}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{pack}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{'['}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisData{[']']}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sa}\KatlaSpace{}\IdrisBound{sb}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{List}\KatlaSpace{}\IdrisType{Char}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{List}\KatlaSpace{}\IdrisType{Char}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{id}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{.}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{'1'::}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{go}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{.}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{'0'::}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisType{Thable}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Any}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisBound{psx}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisBound{psx}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisBound{psx}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Here}\KatlaSpace{}\IdrisBound{px}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{Here}\KatlaSpace{}\IdrisBound{px}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{There}\KatlaSpace{}\IdrisBound{psx}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{There}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{psx}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{th}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{There}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{psx}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{th}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisType{Selable}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{All}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{^?}\KatlaSpace{}\IdrisBound{psy}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{[<]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{psy}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{py}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{psy}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{^?}\KatlaSpace{}\IdrisBound{psy}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{py}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{psy}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{py}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{psy}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{^?}\KatlaSpace{}\IdrisBound{psy}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Properties}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Smart}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{keepInjective}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisFunction{keep}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{ph}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{keepInjective}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{q}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{eq}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{pred}\KatlaSpace{}\IdrisFunction{.}\KatlaSpace{}\IdrisFunction{bigEnd}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{eq}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{keepInjective}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{q}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{consInjective}\KatlaSpace{}\IdrisData{True}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cong}\KatlaSpace{}\IdrisFunction{encoding}\KatlaSpace{}\IdrisBound{eq}\IdrisKeyword{))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{keepInjective}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{q}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Refl}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{irrelevantInvariant}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{q}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{dropInjective}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisFunction{drop}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{ph}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{dropInjective}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{q}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{eq}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{pred}\KatlaSpace{}\IdrisFunction{.}\KatlaSpace{}\IdrisFunction{bigEnd}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{eq}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{dropInjective}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{q}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{shiftLInjective}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cong}\KatlaSpace{}\IdrisFunction{encoding}\KatlaSpace{}\IdrisBound{eq}\IdrisKeyword{))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{dropInjective}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{q}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Refl}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{irrelevantInvariant}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{q}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{mapReflects}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisType{<=>}\KatlaSpace{}\IdrisBound{q}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Reflects}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Reflects}\KatlaSpace{}\IdrisBound{q}\KatlaSpace{}\IdrisBound{b}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{mapReflects}\KatlaSpace{}\IdrisBound{pq}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{RTrue}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{RTrue}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{leftToRight}\KatlaSpace{}\IdrisBound{pq}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{mapReflects}\KatlaSpace{}\IdrisBound{pq}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{RFalse}\KatlaSpace{}\IdrisBound{np}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{RFalse}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{np}\KatlaSpace{}\IdrisFunction{.}\KatlaSpace{}\IdrisFunction{rightToLeft}\KatlaSpace{}\IdrisBound{pq}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{symmetric}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisType{<=>}\KatlaSpace{}\IdrisBound{q}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{q}\KatlaSpace{}\IdrisType{<=>}\KatlaSpace{}\IdrisBound{p}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{symmetric}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkEquivalence}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{g}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkEquivalence}\KatlaSpace{}\IdrisBound{g}\KatlaSpace{}\IdrisBound{f}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{reflectsEquiv}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisType{<=>}\KatlaSpace{}\IdrisBound{q}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Reflects}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisType{<=>}\KatlaSpace{}\IdrisType{Reflects}\KatlaSpace{}\IdrisBound{q}\KatlaSpace{}\IdrisBound{b}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{reflectsEquiv}\KatlaSpace{}\IdrisBound{pq}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkEquivalence}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{mapReflects}\KatlaSpace{}\IdrisBound{pq}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{mapReflects}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{symmetric}\KatlaSpace{}\IdrisBound{pq}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{andReflects}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Reflects}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Reflects}\KatlaSpace{}\IdrisBound{q}\KatlaSpace{}\IdrisBound{c}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Reflects}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{p}\IdrisType{,}\KatlaSpace{}\IdrisBound{q}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{b}\KatlaSpace{}\IdrisFunction{\&\&}\KatlaSpace{}\IdrisBound{c}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{andReflects}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{RTrue}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{RTrue}\KatlaSpace{}\IdrisBound{q}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{RTrue}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{p}\IdrisData{,}\KatlaSpace{}\IdrisBound{q}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{andReflects}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{RTrue}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{RFalse}\KatlaSpace{}\IdrisBound{nq}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{RFalse}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{nq}\KatlaSpace{}\IdrisFunction{.}\KatlaSpace{}\IdrisFunction{snd}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{andReflects}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{RFalse}\KatlaSpace{}\IdrisBound{np}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{rq}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{RFalse}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{np}\KatlaSpace{}\IdrisFunction{.}\KatlaSpace{}\IdrisFunction{fst}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{orReflects}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Reflects}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Reflects}\KatlaSpace{}\IdrisBound{q}\KatlaSpace{}\IdrisBound{c}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Reflects}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Either}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{q}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{b}\KatlaSpace{}\IdrisFunction{||}\KatlaSpace{}\IdrisBound{c}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{orReflects}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{RTrue}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{RTrue}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Left}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{orReflects}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{RFalse}\KatlaSpace{}\IdrisBound{np}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{RTrue}\KatlaSpace{}\IdrisBound{q}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{RTrue}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Right}\KatlaSpace{}\IdrisBound{q}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{orReflects}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{RFalse}\KatlaSpace{}\IdrisBound{np}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{RFalse}\KatlaSpace{}\IdrisBound{nq}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{RFalse}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{either}\KatlaSpace{}\IdrisBound{np}\KatlaSpace{}\IdrisBound{nq}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{reflectsNat}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{m}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Reflects}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{m}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{m}\KatlaSpace{}\IdrisFunction{==}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{reflectsNat}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{RTrue}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{reflectsNat}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{})}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{RFalse}\KatlaSpace{}\IdrisFunction{absurd}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{reflectsNat}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{})}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{RFalse}\KatlaSpace{}\IdrisFunction{absurd}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{reflectsNat}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{m}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{mapReflects}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkEquivalence}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cong}\KatlaSpace{}\IdrisData{S}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{injective}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{reflectsNat}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisBound{n}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Boolean\KatlaSpace{}equality\KatlaSpace{}of\KatlaSpace{}integers\KatlaSpace{}reflects\KatlaSpace{}their\KatlaSpace{}propositional\KatlaSpace{}equality}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}We\KatlaSpace{}can\KatlaSpace{}prove\KatlaSpace{}this\KatlaSpace{}thanks\KatlaSpace{}to\KatlaSpace{}the\KatlaSpace{}fact\KatlaSpace{}that\KatlaSpace{}DecEq\KatlaSpace{}for\KatlaSpace{}Integers\KatlaSpace{}is\KatlaSpace{}implemented}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}using\KatlaSpace{}boolean\KatlaSpace{}equality}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{reflectsInteger}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Reflects}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{==}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{reflectsInteger}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{decEq}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{proof}\KatlaSpace{}\IdrisBound{eq}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{==}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{reflectsInteger}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Yes}\KatlaSpace{}\IdrisBound{prf}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{True}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{RTrue}\KatlaSpace{}\IdrisBound{prf}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{reflectsInteger}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{No}\KatlaSpace{}\IdrisBound{nprf}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{False}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{RFalse}\KatlaSpace{}\IdrisBound{nprf}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{ThEqEquiv}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\IdrisFunction{.bigEnd}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{ph}\IdrisFunction{.bigEnd}\IdrisType{,}\KatlaSpace{}\IdrisBound{th}\IdrisFunction{.encoding}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{ph}\IdrisFunction{.encoding}\IdrisKeyword{)}\KatlaSpace{}\IdrisType{<=>}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{ph}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{ThEqEquiv}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{q}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkEquivalence}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{uncurry}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisData{Refl}\IdrisKeyword{,}\KatlaSpace{}\IdrisData{Refl}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{irrelevantInvariant}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{q}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisData{Refl}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(\textbackslash{}}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cong}\KatlaSpace{}\IdrisFunction{bigEnd}\KatlaSpace{}\IdrisBound{eq}\IdrisData{,}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisFunction{encoding}\KatlaSpace{}\IdrisBound{eq}\IdrisKeyword{))}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{eqReflects}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Reflects}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{==}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{eqReflects}\KatlaSpace{}\IdrisBound{th}\IdrisKeyword{@(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{@(}\IdrisData{MkTh}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{q}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{mapReflects}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{ThEqEquiv}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{andReflects}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{reflectsNat}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{j}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{reflectsInteger}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}If\KatlaSpace{}we\KatlaSpace{}know\KatlaSpace{}there's\KatlaSpace{}a\KatlaSpace{}boolean\KatlaSpace{}that\KatlaSpace{}reflects\KatlaSpace{}a\KatlaSpace{}type\KatlaSpace{}then\KatlaSpace{}the\KatlaSpace{}type\KatlaSpace{}is\KatlaSpace{}decidable}\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{toDec}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Reflects}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Dec}\KatlaSpace{}\IdrisBound{p}\KatlaNewline{}
\IdrisFunction{toDec}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{RTrue}\KatlaSpace{}\IdrisBound{yes}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Yes}\KatlaSpace{}\IdrisBound{yes}\KatlaNewline{}
\IdrisFunction{toDec}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{RFalse}\KatlaSpace{}\IdrisBound{no}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{No}\KatlaSpace{}\IdrisBound{no}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}As\KatlaSpace{}a\KatlaSpace{}consequence\KatlaSpace{}equality\KatlaSpace{}of\KatlaSpace{}thinnings\KatlaSpace{}is\KatlaSpace{}decidable}\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisType{DecEq}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{decEq}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{toDec}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{eqReflects}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Empty\KatlaSpace{}and\KatlaSpace{}identity\KatlaSpace{}thinnings}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Smart}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Empty\KatlaSpace{}thinning}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{--\KatlaSpace{}TODO:\KatlaSpace{}only\KatlaSpace{}take\KatlaSpace{}the\KatlaSpace{}length\KatlaSpace{}as\KatlaSpace{}an\KatlaSpace{}argument?}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*none>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{none}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisData{[<]}\KatlaSpace{}\IdrisBound{sy}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{none}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkTh}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{length}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{none}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</none>
\begin{code}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Identity\KatlaSpace{}thinning}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{--\KatlaSpace{}TODO:\KatlaSpace{}only\KatlaSpace{}take\KatlaSpace{}the\KatlaSpace{}length\KatlaSpace{}as\KatlaSpace{}an\KatlaSpace{}argument?}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*ones>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{ones}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sx}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{ones}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisFunction{n}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat};\KatlaSpace{}\IdrisFunction{n}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{length}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisData{MkTh}\KatlaSpace{}\IdrisFunction{n}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{full}\KatlaSpace{}\IdrisFunction{n}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{ones}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</ones>
\begin{code}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}And\KatlaSpace{}their\KatlaSpace{}properties}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{tooBig}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{Not}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Th}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sx}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{tooBig}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{tooBig}\KatlaSpace{}\IdrisBound{th}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{tooBig}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{drop}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{ones}\KatlaSpace{}?\IdrisKeyword{)}\KatlaSpace{}?\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{th}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{irrelevantNone}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisData{[<]}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{ph}\KatlaNewline{}
\IdrisFunction{irrelevantNone}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{irrelevantDone}\KatlaSpace{}?\KatlaSpace{}?\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`drop`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{irrelevantNone}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{noneIsDrop}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{none}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sx}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisFunction{drop}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{none}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\IdrisFunction{noneIsDrop}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{irrelevantEq}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{irrelevantNone}\KatlaSpace{}?\KatlaSpace{}?\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{irrelevantOnes}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{ph}\KatlaNewline{}
\IdrisFunction{irrelevantOnes}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{irrelevantDone}\KatlaSpace{}?\KatlaSpace{}?\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`keep`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{irrelevantOnes}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{void}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{tooBig}\KatlaSpace{}\IdrisBound{ph}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{void}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{tooBig}\KatlaSpace{}\IdrisBound{th}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{onesIsKeep}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{})}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisFunction{ones}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sx}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisFunction{keep}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{ones}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\IdrisFunction{onesIsKeep}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{irrelevantEq}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{irrelevantOnes}\KatlaSpace{}?\KatlaSpace{}?\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{onesLeftNeutral}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{ph}\KatlaNewline{}
\IdrisFunction{onesLeftNeutral}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{onesLeftNeutral}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{irrelevantDone}\KatlaSpace{}?\KatlaSpace{}?\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{onesLeftNeutral}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{th}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{onesLeftNeutral}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`keep`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{onesLeftNeutral}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{onesLeftNeutral}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{void}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{tooBig}\KatlaSpace{}\IdrisBound{th}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{onesLeftNeutral}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`drop`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{onesLeftNeutral}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{onesRightNeutral}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{th}\KatlaNewline{}
\IdrisFunction{onesRightNeutral}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{onesRightNeutral}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{onesRightNeutral}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{th}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{onesRightNeutral}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`keep`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{onesRightNeutral}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{onesRightNeutral}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`drop`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{onesRightNeutral}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{onesRightNeutral}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{void}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{tooBig}\KatlaSpace{}\IdrisBound{ph}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{transAssoc}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{sw}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ps}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisBound{sz}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{((}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{ps}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ph}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{ps}\IdrisKeyword{))}\KatlaNewline{}
\IdrisFunction{transAssoc}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{ps}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ps}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{transAssoc}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{irrelevantDone}\KatlaSpace{}?\KatlaSpace{}?\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{transAssoc}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ps}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{transAssoc}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ps}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{th}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{transAssoc}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ps}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{viewKeepUnfold}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ph}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{ps}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{viewKeepUnfold}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{viewKeepUnfold}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`keep`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{transAssoc}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{ps}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{transAssoc}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ps}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{viewKeepUnfold}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ph}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{ps}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{viewDropUnfold}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{viewDropUnfold}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`drop`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{transAssoc}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{ps}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{transAssoc}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ps}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{viewDropUnfold}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ph}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{ps}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{viewDropUnfold}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`drop`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{transAssoc}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{ps}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{transAssoc}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{ps}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{viewDropUnfold}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ph}\KatlaSpace{}\IdrisFunction{*^}\KatlaSpace{}\IdrisBound{ps}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`drop`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{transAssoc}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{ps}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Intersection\KatlaSpace{}\&\KatlaSpace{}union\KatlaSpace{}of\KatlaSpace{}supports}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Smart}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{meet}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sxl}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sxr}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Exists}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{`Th`}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{meet}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{thr}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Evidence}\KatlaSpace{}?\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisData{MkTh}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{thl}\KatlaSpace{}\IdrisFunction{.bigEnd}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{thl}\KatlaSpace{}\IdrisFunction{.encoding}\KatlaSpace{}\IdrisFunction{.\&.}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisFunction{.encoding}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{snd}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{Internal.meet}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{thl}\KatlaSpace{}\IdrisFunction{.invariant}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{irrelevantSize}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{thl}\KatlaSpace{}\IdrisFunction{.invariant}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{thr}\KatlaSpace{}\IdrisFunction{.invariant}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisFunction{.invariant}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Meet\KatlaSpace{}is\KatlaSpace{}indeed\KatlaSpace{}computing\KatlaSpace{}a\KatlaSpace{}lower\KatlaSpace{}bound}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}TODO:\KatlaSpace{}prove\KatlaSpace{}it\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}largest\KatlaSpace{}such}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{isMeet}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sxl}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sxr}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Th}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fst}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{meet}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{sxl}\IdrisType{,}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fst}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{meet}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{sxr}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{isMeet}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{done}\IdrisData{,}\KatlaSpace{}\IdrisFunction{done}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{bimap}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`keep`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`keep`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{isMeet}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{mapFst}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`drop`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{isMeet}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{mapSnd}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`drop`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{isMeet}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{isMeet}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{join}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sxl}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sxr}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Exists}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{`Th`}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{join}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{thr}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Evidence}\KatlaSpace{}?\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisData{MkTh}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{thl}\KatlaSpace{}\IdrisFunction{.bigEnd}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{thl}\KatlaSpace{}\IdrisFunction{.encoding}\KatlaSpace{}\IdrisFunction{.|.}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisFunction{.encoding}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{snd}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{Internal.join}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{thl}\KatlaSpace{}\IdrisFunction{.invariant}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{irrelevantSize}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{thl}\KatlaSpace{}\IdrisFunction{.invariant}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{thr}\KatlaSpace{}\IdrisFunction{.invariant}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisFunction{.invariant}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisComment{|||\KatlaSpace{}Join\KatlaSpace{}is\KatlaSpace{}indeed\KatlaSpace{}computing\KatlaSpace{}an\KatlaSpace{}upper\KatlaSpace{}bound}\KatlaNewline{}
\IdrisComment{\KatlaSpace{}\KatlaSpace{}|||\KatlaSpace{}TODO:\KatlaSpace{}prove\KatlaSpace{}it\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}smallest\KatlaSpace{}such}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{isJoin}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sxl}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sxr}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sxl}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fst}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{join}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\IdrisType{,}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sxr}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{fst}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{join}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{isJoin}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{done}\IdrisData{,}\KatlaSpace{}\IdrisFunction{done}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{bimap}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`keep`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`keep`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{isJoin}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{bimap}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`keep`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`drop`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{isJoin}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisKeyword{case}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisKeyword{of}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{bimap}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`drop`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`keep`}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{isJoin}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{isJoin}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{ph}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}Concatenate\KatlaSpace{}two\KatlaSpace{}thinnings}\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{(++)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sa}\KatlaSpace{}\IdrisBound{sb}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sa}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sb}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaNewline{}
\IdrisBound{thl}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkTh}\KatlaSpace{}?\KatlaSpace{}?\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{thl}\IdrisFunction{.invariant}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisBound{thr}\IdrisFunction{.invariant}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}Like\KatlaSpace{}filter\KatlaSpace{}but\KatlaSpace{}returns\KatlaSpace{}a\KatlaSpace{}thinning}\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*which>
\begin{code}
\IdrisFunction{which}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Bool}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{(}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisType{**}\KatlaSpace{}\IdrisType{Th}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisType{)}\KatlaNewline{}
\IdrisFunction{which}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisData{[<]}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}(\IdrisData{[<]}\KatlaSpace{}\IdrisData{**}\KatlaSpace{}\IdrisFunction{done})\KatlaNewline{}
\IdrisFunction{which}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sy}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{y}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}(\IdrisBound{sx}\KatlaSpace{}\IdrisData{**}\KatlaSpace{}\IdrisBound{th})\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{which}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{if}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{y}\KatlaSpace{}\IdrisKeyword{then}\KatlaSpace{}(\IdrisBound{sx}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{y}\KatlaSpace{}\IdrisData{**}\KatlaSpace{}\IdrisFunction{keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{y})\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{else}\KatlaSpace{}(\IdrisBound{sx}\KatlaSpace{}\IdrisData{**}\KatlaSpace{}\IdrisFunction{drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{y})\KatlaNewline{}
\end{code}
%</which>
{-
test : List (sx : SnocList Nat ** Th sx ([<] <>< [0..10]))
test = flip map [2..5] $ \ i =>
        which (\ n => n `mod` i /= 0) ([<] <>< [0..10])
-}
\end{code}



==> Thin/Internal.idr.tex <==

\begin{code}
\IdrisComment{|||\KatlaSpace{}This\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}low-level\KatlaSpace{}stuff\KatlaSpace{}used\KatlaSpace{}to\KatlaSpace{}implement\KatlaSpace{}Thin.}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}The\KatlaSpace{}even\KatlaSpace{}lower\KatlaSpace{}level\KatlaSpace{}(sometimes\KatlaSpace{}unsafe)\KatlaSpace{}results\KatlaSpace{}are\KatlaSpace{}in\KatlaSpace{}Data.Bits.Integer}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{module}\KatlaSpace{}\IdrisModule{Thin.Internal}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Bool}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Bits}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Bits.Integer}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.DPair}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Nat}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.SnocList}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.SnocList.AtIndex}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{\%default}\KatlaSpace{}\IdrisKeyword{total}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}TODO:\KatlaSpace{}move\KatlaSpace{}to\KatlaSpace{}stdlib}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{irrelevantSo}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{q}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{q}\KatlaNewline{}
\IdrisFunction{irrelevantSo}\KatlaSpace{}\IdrisData{Oh}\KatlaSpace{}\IdrisData{Oh}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Thinning\KatlaSpace{}invariant}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}Inductive\KatlaSpace{}relation\KatlaSpace{}characterising\KatlaSpace{}when\KatlaSpace{}a\KatlaSpace{}pair\KatlaSpace{}(i,\KatlaSpace{}bs)\KatlaSpace{}defines\KatlaSpace{}a\KatlaSpace{}thinning}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}@\KatlaSpace{}sx\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}small\KatlaSpace{}end\KatlaSpace{}of\KatlaSpace{}the\KatlaSpace{}thinning}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}@\KatlaSpace{}sy\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}big\KatlaSpace{}end\KatlaSpace{}of\KatlaSpace{}the\KatlaSpace{}thinning}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}@\KatlaSpace{}i\KatlaSpace{}\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}size\KatlaSpace{}of\KatlaSpace{}the\KatlaSpace{}big\KatlaSpace{}end\KatlaSpace{}of\KatlaSpace{}the\KatlaSpace{}thinning}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}@\KatlaSpace{}bs\KatlaSpace{}is\KatlaSpace{}an\KatlaSpace{}integer\KatlaSpace{}but\KatlaSpace{}we\KatlaSpace{}are\KatlaSpace{}only\KatlaSpace{}interested\KatlaSpace{}in\KatlaSpace{}its\KatlaSpace{}first\KatlaSpace{}@i\KatlaSpace{}bits.}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}Each\KatlaSpace{}bit\KatlaSpace{}in\KatlaSpace{}bs\KatlaSpace{}indicates\KatlaSpace{}whether\KatlaSpace{}the\KatlaSpace{}associated\KatlaSpace{}value\KatlaSpace{}in\KatlaSpace{}sy\KatlaSpace{}is\KatlaSpace{}kept\KatlaSpace{}in\KatlaSpace{}sx}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}For\KatlaSpace{}instance:\KatlaSpace{}Invariant\KatlaSpace{}2\KatlaSpace{}[01]\KatlaSpace{}[<y]\KatlaSpace{}[<x,y]\KatlaSpace{}because:}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}i.\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}2\KatlaSpace{}is\KatlaSpace{}the\KatlaSpace{}size\KatlaSpace{}of\KatlaSpace{}[01]\KatlaSpace{}(and\KatlaSpace{}[<x,y])}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}ii.\KatlaSpace{}\KatlaSpace{}[01]\KatlaSpace{}describes\KatlaSpace{}[<y]\KatlaSpace{}as\KatlaSpace{}[<x,y]\KatlaSpace{}where\KatlaSpace{}x\KatlaSpace{}was\KatlaSpace{}discarded\KatlaSpace{}and\KatlaSpace{}y\KatlaSpace{}kept}\KatlaNewline{}
\IdrisComment{|||}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}Doc\KatlaSpace{}for\KatlaSpace{}constructors:}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}A\KatlaSpace{}0-bits\KatlaSpace{}long\KatlaSpace{}thinning\KatlaSpace{}is\KatlaSpace{}a\KatlaSpace{}thinning\KatlaSpace{}between\KatlaSpace{}empty\KatlaSpace{}lists}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}If\KatlaSpace{}the\KatlaSpace{}last\KatlaSpace{}bit\KatlaSpace{}of\KatlaSpace{}interest\KatlaSpace{}is\KatlaSpace{}set\KatlaSpace{}then\KatlaSpace{}the\KatlaSpace{}snoclist's\KatlaSpace{}head\KatlaSpace{}is\KatlaSpace{}kept}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}If\KatlaSpace{}the\KatlaSpace{}last\KatlaSpace{}bit\KatlaSpace{}of\KatlaSpace{}interest\KatlaSpace{}is\KatlaSpace{}not\KatlaSpace{}set\KatlaSpace{}then\KatlaSpace{}the\KatlaSpace{}snoclist's\KatlaSpace{}head\KatlaSpace{}is\KatlaSpace{}thrown\KatlaSpace{}out}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*thinning>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sx}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisData{[<]}\KatlaSpace{}\IdrisData{[<]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{auto}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{Z}\IdrisKeyword{)\}}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sx}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sy}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{auto}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{nb}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{not}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{Z}\IdrisKeyword{))\}}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sy}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</thinning>
\begin{code}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Properties\KatlaSpace{}of\KatlaSpace{}Invariant}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{irrelevantSize}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{sa}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{sb}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{j}\KatlaNewline{}
\IdrisFunction{irrelevantSize}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\IdrisFunction{irrelevantSize}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{irrelevantSize}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{thr}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{irrelevantSize}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{irrelevantSize}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{thr}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{irrelevantSize}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{irrelevantSize}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{thr}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{irrelevantSize}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{irrelevantSize}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{thr}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}The\KatlaSpace{}thinning\KatlaSpace{}relation\KatlaSpace{}is\KatlaSpace{}a\KatlaSpace{}mere\KatlaSpace{}validation\KatlaSpace{}relation\KatlaSpace{}and\KatlaSpace{}thus\KatlaSpace{}entirely}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}characterised\KatlaSpace{}by\KatlaSpace{}its\KatlaSpace{}indices.\KatlaSpace{}Consequently\KatlaSpace{}its\KatlaSpace{}proofs\KatlaSpace{}are\KatlaSpace{}irrelevant.}\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{irrelevantInvariant}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th1}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{th2}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{th1}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{th2}\KatlaNewline{}
\IdrisFunction{irrelevantInvariant}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\IdrisFunction{irrelevantInvariant}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th1}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{b1}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th2}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{b2}\IdrisKeyword{\})}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{cong2}\KatlaSpace{}\IdrisKeyword{(\textbackslash{}}\KatlaSpace{}\IdrisBound{th}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{b}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{irrelevantInvariant}\KatlaSpace{}\IdrisBound{th1}\KatlaSpace{}\IdrisBound{th2}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{irrelevantSo}\KatlaSpace{}\IdrisBound{b1}\KatlaSpace{}\IdrisBound{b2}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{irrelevantInvariant}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th1}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{nb}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{nb1}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th2}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{nb}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{nb2}\IdrisKeyword{\})}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{cong2}\KatlaSpace{}\IdrisKeyword{(\textbackslash{}}\KatlaSpace{}\IdrisBound{th}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{nb}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{nb}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{irrelevantInvariant}\KatlaSpace{}\IdrisBound{th1}\KatlaSpace{}\IdrisBound{th2}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{irrelevantSo}\KatlaSpace{}\IdrisBound{nb1}\KatlaSpace{}\IdrisBound{nb2}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{irrelevantInvariant}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th1}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{b1}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th2}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{nb}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{nb2}\IdrisKeyword{\})}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{void}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{soNotToNotSo}\KatlaSpace{}\IdrisBound{nb2}\KatlaSpace{}\IdrisBound{b1}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{irrelevantInvariant}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th1}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{nb}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{nb1}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th2}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{b2}\IdrisKeyword{\})}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{void}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{soNotToNotSo}\KatlaSpace{}\IdrisBound{nb1}\KatlaSpace{}\IdrisBound{b2}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*none>
\begin{code}
\IdrisFunction{none}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{length}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisData{[<]}\KatlaSpace{}\IdrisBound{sy}\KatlaNewline{}
\IdrisFunction{none}\KatlaSpace{}\IdrisData{[<]}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Done}\KatlaNewline{}
\IdrisFunction{none}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sy}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{y}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{none}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{y}\KatlaNewline{}
\end{code}
%</none>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*ones>
\begin{code}
\IdrisFunction{ones}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{length}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{full}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sx}\KatlaNewline{}
\IdrisFunction{ones}\KatlaSpace{}\IdrisData{[<]}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Done}\KatlaNewline{}
\IdrisFunction{ones}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sx}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{nb}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{eqToSo}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBitFull}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{length}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{))}\KatlaSpace{}\IdrisData{Z}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{shiftRFull}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{length}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisFunction{ones}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\end{code}
%</ones>
\begin{code}
\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}We\KatlaSpace{}need\KatlaSpace{}to\KatlaSpace{}public\KatlaSpace{}export\KatlaSpace{}so\KatlaSpace{}that\KatlaSpace{}`fst\KatlaSpace{}(meet\KatlaSpace{}th\KatlaSpace{}ph)`\KatlaSpace{}computes\KatlaSpace{}at\KatlaSpace{}the\KatlaSpace{}type\KatlaSpace{}level.}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}These\KatlaSpace{}are\KatlaSpace{}all\KatlaSpace{}runtime\KatlaSpace{}irrelevant\KatlaSpace{}though\KatlaSpace{}so\KatlaSpace{}their\KatlaSpace{}behaviour\KatlaSpace{}does\KatlaSpace{}not\KatlaSpace{}matter.}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{meet}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{sxl}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{sxr}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Exists}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{sxlr}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.\&.}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{sxlr}\KatlaSpace{}\IdrisBound{sx}\KatlaNewline{}
\IdrisFunction{meet}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Evidence}\KatlaSpace{}?\KatlaSpace{}\IdrisData{Done}\KatlaNewline{}
\IdrisFunction{meet}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{@\{}\IdrisBound{bl}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{@\{}\IdrisBound{br}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{=}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{ih}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{meet}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.\&.}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitAnd}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{andSo}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bl}\IdrisData{,}\KatlaSpace{}\IdrisBound{br}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisData{Evidence}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ih}\KatlaSpace{}\IdrisFunction{.fst}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{shiftRAnd}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{ih}\KatlaSpace{}\IdrisFunction{.snd}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{meet}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{@\{}\IdrisBound{nbr}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{=}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{ih}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{meet}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{nb}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{not}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.\&.}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitAnd}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{notAndIsOr}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisFunction{orSo}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Right}\KatlaSpace{}\IdrisBound{nbr}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisData{Evidence}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ih}\KatlaSpace{}\IdrisFunction{.fst}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{shiftRAnd}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{ih}\KatlaSpace{}\IdrisFunction{.snd}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{meet}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{@\{}\IdrisBound{nbl}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{ih}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{meet}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{nb}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{not}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.\&.}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitAnd}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{notAndIsOr}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisFunction{orSo}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Left}\KatlaSpace{}\IdrisBound{nbl}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisData{Evidence}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ih}\KatlaSpace{}\IdrisFunction{.fst}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{shiftRAnd}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{ih}\KatlaSpace{}\IdrisFunction{.snd}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{meet}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{@\{}\IdrisBound{nbl}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{ih}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{meet}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{nb}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{not}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.\&.}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitAnd}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{notAndIsOr}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisFunction{orSo}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Left}\KatlaSpace{}\IdrisBound{nbl}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisData{Evidence}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ih}\KatlaSpace{}\IdrisFunction{.fst}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{shiftRAnd}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{ih}\KatlaSpace{}\IdrisFunction{.snd}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}We\KatlaSpace{}need\KatlaSpace{}to\KatlaSpace{}public\KatlaSpace{}export\KatlaSpace{}so\KatlaSpace{}that\KatlaSpace{}`fst\KatlaSpace{}(join\KatlaSpace{}th\KatlaSpace{}ph)`\KatlaSpace{}computes\KatlaSpace{}at\KatlaSpace{}the\KatlaSpace{}type\KatlaSpace{}level.}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}These\KatlaSpace{}are\KatlaSpace{}all\KatlaSpace{}runtime\KatlaSpace{}irrelevant\KatlaSpace{}though\KatlaSpace{}so\KatlaSpace{}their\KatlaSpace{}behaviour\KatlaSpace{}does\KatlaSpace{}not\KatlaSpace{}matter.}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{join}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{sxl}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{sxr}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Exists}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{sxlr}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.|.}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{sxlr}\KatlaSpace{}\IdrisBound{sx}\KatlaNewline{}
\IdrisFunction{join}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Evidence}\KatlaSpace{}?\KatlaSpace{}\IdrisData{Done}\KatlaNewline{}
\IdrisFunction{join}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{@\{}\IdrisBound{bl}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{ih}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{join}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.|.}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitOr}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{orSo}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Left}\KatlaSpace{}\IdrisBound{bl}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisData{Evidence}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ih}\KatlaSpace{}\IdrisFunction{.fst}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{shiftROr}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{ih}\KatlaSpace{}\IdrisFunction{.snd}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{join}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{@\{}\IdrisBound{bl}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{ih}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{join}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.|.}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitOr}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{orSo}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Left}\KatlaSpace{}\IdrisBound{bl}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisData{Evidence}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ih}\KatlaSpace{}\IdrisFunction{.fst}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{shiftROr}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{ih}\KatlaSpace{}\IdrisFunction{.snd}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{join}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{@\{}\IdrisBound{br}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{=}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{ih}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{join}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.|.}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitOr}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{orSo}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Right}\KatlaSpace{}\IdrisBound{br}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisData{Evidence}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ih}\KatlaSpace{}\IdrisFunction{.fst}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{shiftROr}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{ih}\KatlaSpace{}\IdrisFunction{.snd}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{join}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{@\{}\IdrisBound{nbl}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{@\{}\IdrisBound{nbr}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{=}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{ih}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{join}\KatlaSpace{}\IdrisBound{thl}\KatlaSpace{}\IdrisBound{thr}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{not}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{.|.}\KatlaSpace{}\IdrisBound{cs}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBitOr}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{notOrIsAnd}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisFunction{andSo}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{nbl}\IdrisData{,}\KatlaSpace{}\IdrisBound{nbr}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisData{Evidence}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{ih}\KatlaSpace{}\IdrisFunction{.fst}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{shiftROr}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisBound{ih}\KatlaSpace{}\IdrisFunction{.snd}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Inversion\KatlaSpace{}principles}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}Simple\KatlaSpace{}observations\KatlaSpace{}about\KatlaSpace{}the\KatlaSpace{}Nat/Integer\KatlaSpace{}indices\KatlaSpace{}of\KatlaSpace{}a\KatlaSpace{}Invariant\KatlaSpace{}are\KatlaSpace{}enough}\KatlaNewline{}
\IdrisComment{--\KatlaSpace{}to\KatlaSpace{}guarantee\KatlaSpace{}a\KatlaSpace{}proof\KatlaSpace{}was\KatlaSpace{}built\KatlaSpace{}using\KatlaSpace{}a\KatlaSpace{}specific\KatlaSpace{}constructor.}\KatlaNewline{}
\IdrisComment{------------------------------------------------------------------------------}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}Characterising\KatlaSpace{}Done-headed\KatlaSpace{}thinnings}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\IdrisKeyword{record}\KatlaSpace{}\IdrisType{IsDone}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{sx}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}constructor\KatlaSpace{}\IdrisData{MkIsDone}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{bsIsZero}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisData{0}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fstIndexIsLin}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisData{[<]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{sndIndexIsLin}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisData{[<]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{invariantIsDone}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{===}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{replace}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{\textbackslash{}}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{sym}\KatlaSpace{}\IdrisBound{bsIsZero}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{replace}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{sym}\KatlaSpace{}\IdrisBound{sndIndexIsLin}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{replace}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{flip}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Invariant}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{[<]}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{sym}\KatlaSpace{}\IdrisBound{fstIndexIsLin}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisData{Done}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}Proof\KatlaSpace{}that\KatlaSpace{}whenever\KatlaSpace{}the\KatlaSpace{}big\KatlaSpace{}end\KatlaSpace{}is\KatlaSpace{}0,\KatlaSpace{}the\KatlaSpace{}thinning\KatlaSpace{}is\KatlaSpace{}Done}\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{isDone}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{IsDone}\KatlaSpace{}\IdrisBound{th}\KatlaNewline{}
\IdrisFunction{isDone}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkIsDone}\KatlaSpace{}\IdrisData{Refl}\KatlaSpace{}\IdrisData{Refl}\KatlaSpace{}\IdrisData{Refl}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}Characterising\KatlaSpace{}Keep-headed\KatlaSpace{}thinnings}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\IdrisKeyword{record}\KatlaSpace{}\IdrisType{IsKeep}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{sx}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit\KatlaSpace{}}\IdrisBound{bs}\IdrisFunction{\KatlaSpace{}Z}\IdrisKeyword{))}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}constructor\KatlaSpace{}\IdrisData{MkIsKeep}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisFunction{fstIndexTail}\IdrisKeyword{,}\KatlaSpace{}\IdrisFunction{sndIndexTail}\IdrisKeyword{,}\KatlaSpace{}\IdrisFunction{keptHead}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}\}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{fstIndexIsSnoc}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{fstIndexTail}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{keptHead}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{sndIndexIsSnoc}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{sndIndexTail}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{keptHead}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{subInvariant}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\IdrisFunction{\KatlaSpace{}`shiftR`\KatlaSpace{}1}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{fstIndexTail}\KatlaSpace{}\IdrisBound{sndIndexTail}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{invariantIsKeep}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{===}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{replace}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{sym}\KatlaSpace{}\IdrisBound{sndIndexIsSnoc}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{replace}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{flip}\KatlaSpace{}\IdrisKeyword{(}\IdrisType{Invariant}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{bs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sndIndexTail}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{keptHead}\IdrisKeyword{)\}}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{sym}\KatlaSpace{}\IdrisBound{fstIndexIsSnoc}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{subInvariant}\KatlaSpace{}\IdrisBound{keptHead}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{isKeepInteger}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{Z}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisFunction{setBit}\KatlaSpace{}\IdrisKeyword{((}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\KatlaNewline{}
\IdrisFunction{isKeepInteger}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{so}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{sym}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{extensionally}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}case}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{transitive}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{soToEq}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{testSetBitSame}\KatlaSpace{}\IdrisKeyword{((}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{Z}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{sym}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{soToEq}\KatlaSpace{}\IdrisBound{so}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{transitive}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testSetBitOther}\KatlaSpace{}\IdrisKeyword{((}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{absurd}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{transitive}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBitSShiftL}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{transitive}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`testBit`}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{shiftL0}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{testBitShiftR}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisBound{i}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}Proof\KatlaSpace{}that\KatlaSpace{}whenever\KatlaSpace{}the\KatlaSpace{}big\KatlaSpace{}end\KatlaSpace{}is\KatlaSpace{}(S\KatlaSpace{}i),\KatlaSpace{}and\KatlaSpace{}the\KatlaSpace{}(S\KatlaSpace{}i)-bit\KatlaSpace{}is\KatlaSpace{}set}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}then\KatlaSpace{}the\KatlaSpace{}thinning\KatlaSpace{}is\KatlaSpace{}Keep-headed}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{isKeep}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{Z}\IdrisKeyword{))}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{IsKeep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{b}\KatlaNewline{}
\IdrisFunction{isKeep}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{nb}\IdrisKeyword{\})}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{void}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{soNotToNotSo}\KatlaSpace{}\IdrisBound{nb}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{isKeep}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{b1}\IdrisKeyword{\})}\KatlaSpace{}\IdrisBound{b2}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkIsKeep}\KatlaSpace{}\IdrisData{Refl}\KatlaSpace{}\IdrisData{Refl}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(\textbackslash{}}\KatlaSpace{}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{b}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{irrelevantSo}\KatlaSpace{}\IdrisBound{b1}\KatlaSpace{}\IdrisBound{b2}\IdrisKeyword{))}\KatlaNewline{}
\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}Characterising\KatlaSpace{}Drop-headed\KatlaSpace{}thinnings}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\IdrisKeyword{record}\KatlaSpace{}\IdrisType{IsDrop}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{sx}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{b}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{not}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{testBit\KatlaSpace{}}\IdrisBound{bs}\IdrisFunction{\KatlaSpace{}Z}\IdrisKeyword{))}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}constructor\KatlaSpace{}\IdrisData{MkIsDrop}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\{0}\KatlaSpace{}\IdrisFunction{sndIndexTail}\IdrisKeyword{,}\KatlaSpace{}\IdrisFunction{keptHead}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}\}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{sndIndexIsSnoc}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{sndIndexTail}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{keptHead}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{subInvariant}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\IdrisFunction{\KatlaSpace{}`shiftR`\KatlaSpace{}1}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sndIndexTail}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{invariantIsDrop}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{===}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{replace}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{p}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{sym}\KatlaSpace{}\IdrisBound{sndIndexIsSnoc}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{subInvariant}\KatlaSpace{}\IdrisBound{keptHead}\KatlaNewline{}
\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}Proof\KatlaSpace{}that\KatlaSpace{}whenever\KatlaSpace{}the\KatlaSpace{}big\KatlaSpace{}end\KatlaSpace{}is\KatlaSpace{}(S\KatlaSpace{}i),\KatlaSpace{}and\KatlaSpace{}the\KatlaSpace{}(S\KatlaSpace{}i)-bit\KatlaSpace{}is\KatlaSpace{}not\KatlaSpace{}set}\KatlaNewline{}
\IdrisComment{|||\KatlaSpace{}then\KatlaSpace{}the\KatlaSpace{}thinning\KatlaSpace{}is\KatlaSpace{}Drop-headed}\KatlaNewline{}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{isDrop}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{nb}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{not}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{Z}\IdrisKeyword{))}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{IsDrop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{nb}\KatlaNewline{}
\IdrisFunction{isDrop}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Keep}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{b}\IdrisKeyword{\})}\KatlaSpace{}\IdrisBound{nb}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{void}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{soNotToNotSo}\KatlaSpace{}\IdrisBound{nb}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaNewline{}
\IdrisFunction{isDrop}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{nb}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{nb1}\IdrisKeyword{\})}\KatlaSpace{}\IdrisBound{nb2}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkIsDrop}\KatlaSpace{}\IdrisData{Refl}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(\textbackslash{}}\KatlaSpace{}\IdrisBound{nb}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{nb}\IdrisKeyword{\})}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{irrelevantSo}\KatlaSpace{}\IdrisBound{nb1}\KatlaSpace{}\IdrisBound{nb2}\IdrisKeyword{))}\KatlaNewline{}
\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{isDropInteger}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{not}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{Z}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{1}\KatlaNewline{}
\IdrisFunction{isDropInteger}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{so}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{sym}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{extensionally}\KatlaSpace{}\$\KatlaSpace{}\IdrisKeyword{\textbackslash{}case}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{transitive}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit0ShiftL}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{transitive}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{sym}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisFunction{not}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{soToEq}\KatlaSpace{}\IdrisBound{so}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{notInvolutive}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{Z}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=>}\KatlaSpace{}\IdrisFunction{transitive}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBitSShiftL}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{transitive}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cong}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{`testBit`}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{shiftL0}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftR`}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{testBitShiftR}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisBound{i}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*bit>
\begin{code}
\IdrisFunction{bit}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{\}}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{AtIndex}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{length}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{bit}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{[<}\IdrisBound{x}\IdrisData{]}\KatlaSpace{}\IdrisBound{sx}\KatlaNewline{}
\IdrisFunction{bit}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{none}\KatlaSpace{}?\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\IdrisFunction{bit}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{let}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisBound{nb}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{So}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{not}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{the}\KatlaSpace{}\IdrisType{Integer}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{bit}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{eqToSo}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{cong}\KatlaSpace{}\IdrisFunction{not}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{testBit0ShiftL}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{pred}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{shiftRBitS}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{pred}\KatlaSpace{}\IdrisBound{i}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaSpace{}\IdrisFunction{bit}\KatlaSpace{}\IdrisBound{p}\IdrisKeyword{)}\KatlaSpace{}?\KatlaNewline{}
\end{code}
%</bit>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\IdrisFunction{(++)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{sa}\KatlaSpace{}\IdrisBound{sb}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{Invariant}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{i}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{j}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{cs}\KatlaSpace{}\IdrisFunction{.|.}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisBound{j}\IdrisKeyword{))}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sa}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisBound{sx}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sb}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisBound{sy}\IdrisKeyword{)}\KatlaNewline{}
\IdrisBound{th}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisData{Done}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{plusZeroRightNeutral}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{shiftL0}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{orZeroBitsLeftIdentity}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{th}\KatlaNewline{}
\IdrisBound{th}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{j}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{@\{}\IdrisBound{so}\IdrisKeyword{\}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{sym}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{plusSuccRightSucc}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{shiftROr}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisBound{j}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{shiftLSR}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{@\{rewrite}\KatlaSpace{}\IdrisFunction{testBitOr}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisBound{j}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBit0ShiftL}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{orFalseNeutral}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{Z}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{so}\IdrisKeyword{\}}\KatlaNewline{}
\IdrisBound{th}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{i}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{j}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{ph}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{@\{}\IdrisBound{soNot}\IdrisKeyword{\}}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{sym}\KatlaSpace{}\$\KatlaSpace{}\IdrisFunction{plusSuccRightSucc}\KatlaSpace{}\IdrisBound{i}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{(rewrite}\KatlaSpace{}\IdrisFunction{shiftROr}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisBound{j}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{1}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{shiftLSR}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{th}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisBound{ph}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{x}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{@\{rewrite}\KatlaSpace{}\IdrisFunction{testBitOr}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{bs}\KatlaSpace{}\IdrisFunction{`shiftL`}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisBound{j}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{testBit0ShiftL}\KatlaSpace{}\IdrisBound{bs}\KatlaSpace{}\IdrisBound{j}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{rewrite}\KatlaSpace{}\IdrisFunction{orFalseNeutral}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{testBit}\KatlaSpace{}\IdrisKeyword{\{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisType{Integer}\IdrisKeyword{\}}\KatlaSpace{}\IdrisBound{cs}\KatlaSpace{}\IdrisData{Z}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{in}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisBound{soNot}\IdrisKeyword{\}}\KatlaNewline{}
\end{code}



==> Thinnings.idr.tex <==

\begin{code}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Family}\KatlaNewline{}
\end{code}
%<*family>
\begin{code}
\KatlaSpace{}\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Thinning}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sx}\IdrisKeyword{,}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{SnocList}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Thinning}\KatlaSpace{}\IdrisData{[<]}\KatlaSpace{}\IdrisData{[<]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Thinning}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Thinning}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sx}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sy}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Thinning}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisBound{sy}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(0}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Thinning}\KatlaSpace{}\IdrisBound{sx}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{sy}\KatlaSpace{}\IdrisData{:<}\KatlaSpace{}\IdrisBound{x}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</family>

\begin{code}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Bare}\KatlaNewline{}
\end{code}
%<*bare>
\begin{code}
\KatlaSpace{}\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Thinning}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Done}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Keep}\KatlaSpace{}\IdrisType{Thinning}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Drop}\KatlaSpace{}\IdrisType{Thinning}\KatlaNewline{}
\end{code}
%</bare>



==> UTLC.idr.tex <==

\begin{code}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{Data.Fin}\KatlaNewline{}
\end{code}

%<*term>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{Tm}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Var}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Fin}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Tm}\KatlaSpace{}\IdrisBound{n}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Lam}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Tm}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Tm}\KatlaSpace{}\IdrisBound{n}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{App}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Tm}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Tm}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Tm}\KatlaSpace{}\IdrisBound{n}\KatlaNewline{}
\end{code}
%</term>

%<*scomb>
\begin{code}
\IdrisFunction{scomb}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Tm}\KatlaSpace{}\IdrisData{0}\KatlaNewline{}
\IdrisFunction{scomb}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Lam}\KatlaSpace{}\$\KatlaSpace{}\IdrisData{Lam}\KatlaSpace{}\$\KatlaSpace{}\IdrisData{Lam}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\$\KatlaSpace{}\IdrisData{App}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{App}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Var}\KatlaSpace{}\IdrisData{2}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Var}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{))}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{App}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Var}\KatlaSpace{}\IdrisData{1}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{Var}\KatlaSpace{}\IdrisData{0}\IdrisKeyword{))}\KatlaNewline{}
\end{code}
%</scomb>



==> VectAsList.idr.tex <==

\begin{code}
\IdrisKeyword{module}\KatlaSpace{}\IdrisModule{VectAsList}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{\%default}\KatlaSpace{}\IdrisKeyword{total}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*vect>
\begin{code}
\IdrisKeyword{record}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Type}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}constructor\KatlaSpace{}\IdrisData{MkVect}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{encoding}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{List}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{0}\KatlaSpace{}\IdrisFunction{valid}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisFunction{length}\KatlaSpace{}\IdrisBound{encoding}\KatlaSpace{}\IdrisFunction{===}\KatlaSpace{}\IdrisBound{n}\KatlaNewline{}
\end{code}
%</vect>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Smart}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*nil>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Nil}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{Nil}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkVect}\KatlaSpace{}\IdrisData{[]}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\end{code}
%</nil>

\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*cons>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{(::)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisFunction{::}\KatlaSpace{}\IdrisData{MkVect}\KatlaSpace{}\IdrisBound{xs}\KatlaSpace{}\IdrisBound{eq}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkVect}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{cong}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisBound{eq}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</cons>

\begin{code}
\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*dataview>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{View}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{Nil}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{View}\KatlaSpace{}\IdrisFunction{Nil}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{(::)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{xs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{View}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisFunction{::}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</dataview>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{Smart}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{public}\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*view>
\begin{code}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{xs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{View}\KatlaSpace{}\IdrisBound{xs}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkVect}\KatlaSpace{}\IdrisData{[]}\KatlaSpace{}\IdrisData{Refl}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{Nil}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{view}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{MkVect}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaSpace{}\IdrisData{Refl}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisData{MkVect}\KatlaSpace{}\IdrisBound{xs}\KatlaSpace{}\IdrisData{Refl}\KatlaNewline{}
\end{code}
%</view>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*map>
\begin{code}
\IdrisFunction{map}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisBound{b}\KatlaNewline{}
\IdrisFunction{map}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{@\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{[]}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{[]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisBound{hd}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{tl}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{hd}\KatlaSpace{}\IdrisFunction{::}\KatlaSpace{}\IdrisFunction{map}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{tl}\KatlaNewline{}
\end{code}
%</map>


%<*append>
\begin{code}
\IdrisFunction{(++)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{m}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\IdrisBound{xs}\IdrisKeyword{@\KatlaUnderscore{}}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisBound{ys}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{[]}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{ys}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisBound{hd}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{tl}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{hd}\KatlaSpace{}\IdrisFunction{::}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{tl}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisBound{ys}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</append>
\begin{code}
\KatlaNewline{}
\end{code}
%<*splitAtrel>
\begin{code}
\IdrisKeyword{data}\KatlaSpace{}\IdrisType{SplitAt}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{m}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{xs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{p}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Type}\KatlaSpace{}\IdrisKeyword{where}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisData{MkSplitAt}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{pref}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{suff}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisType{SplitAt}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{pref}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisBound{suff}\IdrisKeyword{)}\KatlaNewline{}
\end{code}
%</splitAtrel>
\begin{code}
\KatlaNewline{}
\IdrisKeyword{namespace}\KatlaSpace{}\IdrisNamespace{SplitAt}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\IdrisKeyword{export}\KatlaNewline{}
\end{code}
%<*splitAtcons>
\begin{code}
\KatlaSpace{}\IdrisFunction{(::)}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{SplitAt}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisBound{xs}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{SplitAt}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{m}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisFunction{::}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\IdrisBound{x}\KatlaSpace{}\IdrisFunction{::}\KatlaSpace{}\IdrisData{MkSplitAt}\KatlaSpace{}\IdrisBound{pref}\IdrisKeyword{@(}\IdrisData{MkVect}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisData{Refl}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{suff}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkSplitAt}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{x}\KatlaSpace{}\IdrisFunction{::}\KatlaSpace{}\IdrisBound{pref}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{suff}\KatlaNewline{}
\end{code}
%</splitAtcons>
\begin{code}
\KatlaNewline{}
\end{code}
%<*splitAtFail1>
\begin{code}
\IdrisKeyword{failing}\KatlaSpace{}\IdrisData{"tl\KatlaSpace{}is\KatlaSpace{}not\KatlaSpace{}accessible\KatlaSpace{}in\KatlaSpace{}this\KatlaSpace{}context"}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{splitAt}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{m}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{xs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{m}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{SplitAt}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisBound{xs}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{splitAt}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisBound{xs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkSplitAt}\KatlaSpace{}\IdrisFunction{[]}\KatlaSpace{}\IdrisBound{xs}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{splitAt}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{m}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{@\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisBound{hd}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{tl}\IdrisKeyword{@\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{splitAt}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}tl\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}res\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}?a\KatlaNewline{}
\end{code}
%</splitAtFail1>
\begin{code}
\KatlaNewline{}
\end{code}
%<*splitAtFail2>
\begin{code}
\IdrisKeyword{failing}\KatlaSpace{}\IdrisData{"Can't\KatlaSpace{}match\KatlaSpace{}on\KatlaSpace{}?postpone\KatlaSpace{}[no\KatlaSpace{}locals\KatlaSpace{}in\KatlaSpace{}scope]\KatlaSpace{}(User\KatlaSpace{}dotted)"}\KatlaNewline{}
\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{splitAt}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{m}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{xs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{m}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{SplitAt}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisBound{xs}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{splitAt}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisBound{xs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkSplitAt}\KatlaSpace{}\IdrisFunction{[]}\KatlaSpace{}\IdrisBound{xs}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{splitAt}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{m}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{@\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisBound{hd}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{tl}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{splitAt}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisBound{tl}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisFunction{splitAt}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{m}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{.(}hd\KatlaSpace{}::\KatlaSpace{}\IdrisKeyword{(}pref\KatlaSpace{}++\KatlaSpace{}suff\IdrisKeyword{))}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisBound{hd}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisKeyword{.(}\IdrisBound{pref}\KatlaSpace{}\IdrisFunction{++}\KatlaSpace{}\IdrisBound{suff}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{MkSplitAt}\KatlaSpace{}\IdrisBound{pref}\KatlaSpace{}\IdrisBound{suff}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}?a\KatlaNewline{}
\end{code}
%</splitAtFail2>
\begin{code}
\KatlaNewline{}
\end{code}
%<*splitAt>
\begin{code}
\IdrisFunction{splitAt}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{m}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Nat}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{xs}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{m}\KatlaSpace{}\IdrisFunction{+}\KatlaSpace{}\IdrisBound{n}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{a}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{SplitAt}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisBound{xs}\KatlaNewline{}
\IdrisFunction{splitAt}\KatlaSpace{}\IdrisData{0}\KatlaSpace{}\IdrisBound{xs}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisData{MkSplitAt}\KatlaSpace{}\IdrisFunction{[]}\KatlaSpace{}\IdrisBound{xs}\KatlaNewline{}
\IdrisFunction{splitAt}\KatlaSpace{}\IdrisKeyword{(}\IdrisData{S}\KatlaSpace{}\IdrisBound{m}\IdrisKeyword{)}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{@\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisKeyword{\KatlaUnderscore{}}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisBound{hd}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{tl}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{hd}\KatlaSpace{}\IdrisFunction{::}\KatlaSpace{}\IdrisFunction{splitAt}\KatlaSpace{}\IdrisBound{m}\KatlaSpace{}\IdrisBound{tl}\KatlaNewline{}
\end{code}
%</splitAt>
\begin{code}



==> WithExpanded.idr.tex <==

\begin{code}
\IdrisKeyword{module}\KatlaSpace{}\IdrisModule{WithExpanded}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{VectAsList}\KatlaNewline{}
\IdrisKeyword{import}\KatlaSpace{}\IdrisModule{FinAsNat}\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{\%hide}\KatlaSpace{}VectAsList.map\KatlaNewline{}
\KatlaNewline{}
\IdrisKeyword{\%default}\KatlaSpace{}\IdrisKeyword{total}\KatlaNewline{}
\KatlaNewline{}
\end{code}
%<*map>
\begin{code}
\IdrisFunction{map}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisKeyword{(}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{b}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisBound{b}\KatlaNewline{}
\IdrisFunction{map}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{xs}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{map}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{.(}\IdrisFunction{[]}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{[]}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{[]}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{map}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisKeyword{.(}\IdrisBound{hd}\KatlaSpace{}\IdrisFunction{::}\KatlaSpace{}\IdrisBound{tl}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisBound{hd}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{tl}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{hd}\KatlaSpace{}\IdrisFunction{::}\KatlaSpace{}\IdrisFunction{map}\KatlaSpace{}\IdrisBound{f}\KatlaSpace{}\IdrisBound{tl}\KatlaNewline{}
\end{code}
%</map>

\end{code}
%<*lookup>
\begin{code}
\IdrisFunction{lookup}\KatlaSpace{}\IdrisKeyword{:}\KatlaSpace{}\IdrisType{Vect}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisBound{a}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisType{Fin}\KatlaSpace{}\IdrisBound{n}\KatlaSpace{}\IdrisKeyword{->}\KatlaSpace{}\IdrisBound{a}\KatlaNewline{}
\IdrisFunction{lookup}\KatlaSpace{}\IdrisBound{xs}\KatlaSpace{}\IdrisBound{k}\KatlaSpace{}\IdrisKeyword{with}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{xs}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisKeyword{(}\IdrisFunction{view}\KatlaSpace{}\IdrisBound{k}\IdrisKeyword{)}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{lookup}\KatlaSpace{}\IdrisKeyword{.(}\IdrisBound{hd}\KatlaSpace{}\IdrisFunction{::}\KatlaSpace{}\IdrisBound{tl}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{.(}\IdrisFunction{Z}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisBound{hd}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{tl}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{Z}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisBound{hd}\KatlaNewline{}
\KatlaSpace{}\KatlaSpace{}\IdrisFunction{lookup}\KatlaSpace{}\IdrisKeyword{.(}\IdrisBound{hd}\KatlaSpace{}\IdrisFunction{::}\KatlaSpace{}\IdrisBound{tl}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{.(}\IdrisFunction{S}\KatlaSpace{}\IdrisBound{k'}\IdrisKeyword{)}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisBound{hd}\KatlaSpace{}\IdrisData{::}\KatlaSpace{}\IdrisBound{tl}\KatlaSpace{}\IdrisKeyword{|}\KatlaSpace{}\IdrisData{S}\KatlaSpace{}\IdrisBound{k'}\KatlaSpace{}\IdrisKeyword{=}\KatlaSpace{}\IdrisFunction{lookup}\KatlaSpace{}\IdrisBound{tl}\KatlaSpace{}\IdrisBound{k'}\KatlaNewline{}
\end{code}
%</lookup>



==> ast.tex <==

%<*named>
\begin{tikzpicture}
\draw (0,0) circle (.3cm) node[align=center] {$\lambda{}g.$};
\draw (2,0) circle (.3cm) node[align=center] {$\lambda{}f.$};
\draw (4,0) circle (.3cm) node[align=center] {$\lambda{}x.$};

\draw (6,0) circle (.3cm) node[align=center] {\$};

\draw (8,1) circle (.3cm) node[align=center] {\$};
\draw (10,1.5) node[align=center] {$g$} +(-.3cm,-.3cm) rectangle +(.3cm,.3cm);
\draw (10,.5)  node[align=center] {$x$} +(-.3cm,-.3cm) rectangle +(.3cm,.3cm);

\draw (8,-1) circle (.3cm) node[align=center] {\$};
\draw (10,-.5)  node[align=center] {$f$} +(-.3cm,-.3cm) rectangle +(.3cm,.3cm);
\draw (10,-1.5) node[align=center] {$x$} +(-.3cm,-.3cm) rectangle +(.3cm,.3cm);

\draw [->] (0.3,0)     to [out=0,in=180]   (1.7,0);
\draw [->] (2.3,0)     to [out=0,in=180]   (3.7,0);
\draw [->] (4.3,0)     to [out=0,in=180]   (5.7,0);
\draw [->] (6.2,-.22)  to [out=-45,in=180]  (7.7,-1);
\draw [->] (6.2,.22)   to [out=45,in=180]  (7.7,1);
\draw [->] (8.2,1.22)  to [out=45,in=180]  (9.7,1.5);
\draw [->] (8.2,.78)   to [out=-45,in=180] (9.7,.5);
\draw [->] (8.2,-1.22) to [out=-45,in=180] (9.7,-1.5);
\draw [->] (8.2,-.78)  to [out=45,in=180]  (9.7,-.5);
\end{tikzpicture}
%</named>

%<*debruijn>
\begin{tikzpicture}
\draw[draw=blue   ,thick] (0,0) circle (.3cm) node[align=center] {$\lambda{}.$};
\draw[draw=magenta,thick] (2,0) circle (.3cm) node[align=center] {$\lambda{}.$};
\draw[draw=orange ,thick] (4,0) circle (.3cm) node[align=center] {$\lambda{}.$};

\draw (6,0) circle (.3cm) node[align=center] {\$};

\draw (8,1) circle (.3cm) node[align=center] {\$};
\draw[fill=blue]   (10,1.5) +(-.3cm,-.3cm) rectangle +(.3cm,.3cm);
\draw[fill=orange] (10,.5)  +(-.3cm,-.3cm) rectangle +(.3cm,.3cm);

\draw (8,-1) circle (.3cm) node[align=center] {\$};
\draw[fill=magenta] (10,-.5)  +(-.3cm,-.3cm) rectangle +(.3cm,.3cm);
\draw[fill=orange]  (10,-1.5) +(-.3cm,-.3cm) rectangle +(.3cm,.3cm);

\draw [->] (0.3,0)     to [out=0,in=180]   (1.7,0);
\draw [->] (2.3,0)     to [out=0,in=180]   (3.7,0);
\draw [->] (4.3,0)     to [out=0,in=180]   (5.7,0);
\draw [->] (6.2,-.22)  to [out=-45,in=180]  (7.7,-1);
\draw [->] (6.2,.22)   to [out=45,in=180]  (7.7,1);
\draw [->] (8.2,1.22)  to [out=45,in=180]  (9.7,1.5);
\draw [->] (8.2,.78)   to [out=-45,in=180] (9.7,.5);
\draw [->] (8.2,-1.22) to [out=-45,in=180] (9.7,-1.5);
\draw [->] (8.2,-.78)  to [out=45,in=180]  (9.7,-.5);

\draw[blue, dotted, thick] [->] (9.7,1.8)   to [out=165,in=45] (0.2,.22);

\draw[orange, thick] [->] (9.7,.8)   to [out=135,in=65] (4,.3);

\draw[magenta, dashed, thick] [->] (9.7,-.2)   to [out=155,in=25] (2.2,.22);

\draw[orange, thick] [->] (9.7,-1.8) to [out=180,in=335] (4.2,-.22);

\end{tikzpicture}
%</debruijn>

%<*codebruijn>
\begin{tikzpicture}
\draw[draw=blue   ,thick] (0,0) circle (.3cm) node[align=center] {$\lambda{}.$};
\draw[draw=magenta,thick] (2,0) circle (.3cm) node[align=center] {$\lambda{}.$};
\draw[draw=orange ,thick] (4,0) circle (.3cm) node[align=center] {$\lambda{}.$};

\draw (6,0) circle (.3cm) node[align=center] {\$};

\draw (8,1)    circle (.3cm) node[align=center] {\$};
\draw[fill=blue]   (10,1.5) +(-.3cm,-.3cm) rectangle +(.3cm,.3cm);
\draw[fill=orange] (10,.5)  +(-.3cm,-.3cm) rectangle +(.3cm,.3cm);

\draw (8,-1)    circle (.3cm) node[align=center] {\$};
\draw[fill=magenta] (10,-.5)  +(-.3cm,-.3cm) rectangle +(.3cm,.3cm);
\draw[fill=orange]  (10,-1.5) +(-.3cm,-.3cm) rectangle +(.3cm,.3cm);


\draw [->] (0.3,0)   to [out=0,in=180] node[above]{$\color{blue}{\bullet}$} (1.7,0);
\draw [->] (2.3,0)   to [out=0,in=180] node[above]{$\color{blue}{\bullet}\color{magenta}{\bullet}$} (3.7,0);
\draw [->] (4.3,0)   to [out=0,in=180] node[above]{$\color{blue}{\bullet}\color{magenta}{\bullet}\color{orange}{\bullet}$} (5.7,0);

\draw [->] (6.2,-.22)  to [out=-45,in=180] node[below left]{$\color{blue}{\circ}\color{magenta}{\bullet}\color{orange}{\bullet}$} (7.7,-1);
\draw [->] (6.2,.22)   to [out=45,in=180] node[above left]{$\color{blue}{\bullet}\color{magenta}{\circ}\color{orange}{\bullet}$} (7.7,1);
\draw [->] (8.2,1.22)  to [out=45,in=180] node[above]{$\color{blue}{\bullet}\color{orange}{\circ}$} (9.7,1.5);
\draw [->] (8.2,.78)   to [out=-45,in=180] node[below]{$\color{blue}{\circ}\color{orange}{\bullet}$} (9.7,.5);
\draw [->] (8.2,-.78)  to [out=45,in=180] node[above]{$\color{magenta}{\bullet}\color{orange}{\circ}$} (9.7,-.5);
\draw [->] (8.2,-1.22) to [out=-45,in=180] node[below]{$\color{magenta}{\circ}\color{orange}{\bullet}$} (9.7,-1.5);
\end{tikzpicture}
%</codebruijn>

%<*opening>
\begin{tikzpicture}
\draw (0,0)     circle (.3cm) node[align=center] {\$};
\draw (2.5,.75)   node[draw,dashed,regular polygon, regular polygon sides=3, shape border rotate=90]{$t_1$};
\draw (2.5,-.75)  node[draw,dashed,regular polygon, regular polygon sides=3, shape border rotate=90]{$t_2$};

\draw (-1,0)
  node[align=center]{$\color{blue}{\bullet}\color{orange}{\circ}\color{magenta}{\bullet}\color{teal}{\bullet}\color{lightgray}{\bullet}$} (1.7,1.5);
\draw [->] (.2,.22)  to [out=45,in=180]
  node[above]{$\color{blue}{\circ}\color{magenta}{\bullet}\color{teal}{\bullet}\color{lightgray}{\circ}$}
  (1.77,.75);
\draw [->] (.2,-.22) to [out=-45,in=180]
  node[below]{$\color{blue}{\bullet}\color{magenta}{\circ}\color{teal}{\bullet}\color{lightgray}{\bullet}$}
  (1.77,-.75);
\end{tikzpicture}
%</opening>

%<*opened>
\begin{tikzpicture}
\draw (0,0)       node[draw,diamond,align=center] {\$};
\draw (2.5,.75)   node[draw,dashed,regular polygon, regular polygon sides=3, shape border rotate=90]{$t_1$};
\draw (2.5,-.75)  node[draw,dashed,regular polygon, regular polygon sides=3, shape border rotate=90]{$t_2$};

\draw [->] (.23,.23)  to [out=45,in=180]
  node[above]{$\color{blue}{\circ}\color{orange}{\circ}\color{magenta}{\bullet}\color{teal}{\bullet}\color{lightgray}{\circ}$}
  (1.77,.75);
\draw [->] (.23,-.23) to [out=-45,in=180]
  node[below]{$\color{blue}{\bullet}\color{orange}{\circ}\color{magenta}{\circ}\color{teal}{\bullet}\color{lightgray}{\bullet}$}
  (1.77,-.75);
\end{tikzpicture}
%</opened>


==> minted-preamble.tex <==

\makeatletter
\def\PYG@reset{\let\PYG@it=\relax \let\PYG@bf=\relax%
    \let\PYG@ul=\relax \let\PYG@tc=\relax%
    \let\PYG@bc=\relax \let\PYG@ff=\relax}
\def\PYG@tok#1{\csname PYG@tok@#1\endcsname}
\def\PYG@toks#1+{\ifx\relax#1\empty\else%
    \PYG@tok{#1}\expandafter\PYG@toks\fi}
\def\PYG@do#1{\PYG@bc{\PYG@tc{\PYG@ul{%
    \PYG@it{\PYG@bf{\PYG@ff{#1}}}}}}}
\def\PYG#1#2{\PYG@reset\PYG@toks#1+\relax+\PYG@do{#2}}

\@namedef{PYG@tok@w}{\def\PYG@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\@namedef{PYG@tok@c}{\let\PYG@it=\textit\def\PYG@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PYG@tok@cp}{\def\PYG@tc##1{\textcolor[rgb]{0.61,0.40,0.00}{##1}}}
\@namedef{PYG@tok@k}{\let\PYG@bf=\textbf\def\PYG@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PYG@tok@kp}{\def\PYG@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PYG@tok@kt}{\def\PYG@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\@namedef{PYG@tok@o}{\def\PYG@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PYG@tok@ow}{\let\PYG@bf=\textbf\def\PYG@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\@namedef{PYG@tok@nb}{\def\PYG@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PYG@tok@nf}{\def\PYG@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PYG@tok@nc}{\let\PYG@bf=\textbf\def\PYG@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PYG@tok@nn}{\let\PYG@bf=\textbf\def\PYG@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PYG@tok@ne}{\let\PYG@bf=\textbf\def\PYG@tc##1{\textcolor[rgb]{0.80,0.25,0.22}{##1}}}
\@namedef{PYG@tok@nv}{\def\PYG@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PYG@tok@no}{\def\PYG@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\@namedef{PYG@tok@nl}{\def\PYG@tc##1{\textcolor[rgb]{0.46,0.46,0.00}{##1}}}
\@namedef{PYG@tok@ni}{\let\PYG@bf=\textbf\def\PYG@tc##1{\textcolor[rgb]{0.44,0.44,0.44}{##1}}}
\@namedef{PYG@tok@na}{\def\PYG@tc##1{\textcolor[rgb]{0.41,0.47,0.13}{##1}}}
\@namedef{PYG@tok@nt}{\let\PYG@bf=\textbf\def\PYG@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PYG@tok@nd}{\def\PYG@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\@namedef{PYG@tok@s}{\def\PYG@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PYG@tok@sd}{\let\PYG@it=\textit\def\PYG@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PYG@tok@si}{\let\PYG@bf=\textbf\def\PYG@tc##1{\textcolor[rgb]{0.64,0.35,0.47}{##1}}}
\@namedef{PYG@tok@se}{\let\PYG@bf=\textbf\def\PYG@tc##1{\textcolor[rgb]{0.67,0.36,0.12}{##1}}}
\@namedef{PYG@tok@sr}{\def\PYG@tc##1{\textcolor[rgb]{0.64,0.35,0.47}{##1}}}
\@namedef{PYG@tok@ss}{\def\PYG@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PYG@tok@sx}{\def\PYG@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PYG@tok@m}{\def\PYG@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PYG@tok@gh}{\let\PYG@bf=\textbf\def\PYG@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\@namedef{PYG@tok@gu}{\let\PYG@bf=\textbf\def\PYG@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\@namedef{PYG@tok@gd}{\def\PYG@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\@namedef{PYG@tok@gi}{\def\PYG@tc##1{\textcolor[rgb]{0.00,0.52,0.00}{##1}}}
\@namedef{PYG@tok@gr}{\def\PYG@tc##1{\textcolor[rgb]{0.89,0.00,0.00}{##1}}}
\@namedef{PYG@tok@ge}{\let\PYG@it=\textit}
\@namedef{PYG@tok@gs}{\let\PYG@bf=\textbf}
\@namedef{PYG@tok@gp}{\let\PYG@bf=\textbf\def\PYG@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\@namedef{PYG@tok@go}{\def\PYG@tc##1{\textcolor[rgb]{0.44,0.44,0.44}{##1}}}
\@namedef{PYG@tok@gt}{\def\PYG@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\@namedef{PYG@tok@err}{\def\PYG@bc##1{{\setlength{\fboxsep}{\string -\fboxrule}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}}
\@namedef{PYG@tok@kc}{\let\PYG@bf=\textbf\def\PYG@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PYG@tok@kd}{\let\PYG@bf=\textbf\def\PYG@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PYG@tok@kn}{\let\PYG@bf=\textbf\def\PYG@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PYG@tok@kr}{\let\PYG@bf=\textbf\def\PYG@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PYG@tok@bp}{\def\PYG@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\@namedef{PYG@tok@fm}{\def\PYG@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\@namedef{PYG@tok@vc}{\def\PYG@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PYG@tok@vg}{\def\PYG@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PYG@tok@vi}{\def\PYG@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PYG@tok@vm}{\def\PYG@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\@namedef{PYG@tok@sa}{\def\PYG@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PYG@tok@sb}{\def\PYG@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PYG@tok@sc}{\def\PYG@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PYG@tok@dl}{\def\PYG@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PYG@tok@s2}{\def\PYG@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PYG@tok@sh}{\def\PYG@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PYG@tok@s1}{\def\PYG@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\@namedef{PYG@tok@mb}{\def\PYG@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PYG@tok@mf}{\def\PYG@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PYG@tok@mh}{\def\PYG@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PYG@tok@mi}{\def\PYG@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PYG@tok@il}{\def\PYG@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PYG@tok@mo}{\def\PYG@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\@namedef{PYG@tok@ch}{\let\PYG@it=\textit\def\PYG@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PYG@tok@cm}{\let\PYG@it=\textit\def\PYG@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PYG@tok@cpf}{\let\PYG@it=\textit\def\PYG@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PYG@tok@c1}{\let\PYG@it=\textit\def\PYG@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}
\@namedef{PYG@tok@cs}{\let\PYG@it=\textit\def\PYG@tc##1{\textcolor[rgb]{0.24,0.48,0.48}{##1}}}

\def\PYGZbs{\char`\\}
\def\PYGZus{\char`\_}
\def\PYGZob{\char`\{}
\def\PYGZcb{\char`\}}
\def\PYGZca{\char`\^}
\def\PYGZam{\char`\&}
\def\PYGZlt{\char`\<}
\def\PYGZgt{\char`\>}
\def\PYGZsh{\char`\#}
\def\PYGZpc{\char`\%}
\def\PYGZdl{\char`\$}
\def\PYGZhy{\char`\-}
\def\PYGZsq{\char`\'}
\def\PYGZdq{\char`\"}
\def\PYGZti{\char`\~}
% for compatibility with earlier versions
\def\PYGZat{@}
\def\PYGZlb{[}
\def\PYGZrb{]}
\makeatother



==> robust-catch.tex <==
\makeatletter

\newrobustcmd*\OrigExecuteMetaData[2][\jobname]{%
\CatchFileBetweenTags\CatchFBT@tok{#1}{#2}%
\global\expandafter\CatchFBT@tok\expandafter{%
\expandafter}\the\CatchFBT@tok
}%\OrigExecuteMetaData

\newrobustcmd*\ChkExecuteMetaData[2][\jobname]{%
\CatchFileBetweenTags\CatchFBT@tok{#1}{#2}%
\edef\mytokens{\detokenize\expandafter{\the\CatchFBT@tok}}
\ifx\mytokens\empty\PackageError{catchfilebetweentags}{the tag #2 is not found\MessageBreak in file #1 \MessageBreak called from \jobname.tex}{use a different tag}\fi%
}%\ChkExecuteMetaData

\renewrobustcmd*\ExecuteMetaData[2][\jobname]{%
\ChkExecuteMetaData[#1]{#2}%
\OrigExecuteMetaData[#1]{#2}%
}

\makeatother

